Snowmass Topical Group Summary Report: IF04 -- Trigger and Data Acquisition Systems

A trend for future high energy physics experiments is an increase in the data bandwidth produced from the detectors. Datasets of the Petabyte scale have already become the norm, and the requirements of future experiments -- greater in size, exposure, and complexity -- will further push the limits of data acquisition technologies to data rates of exabytes per seconds. The challenge for these future data-intensive physics facilities lies in the reduction of the flow of data through a combination of sophisticated event selection in the form of high-performance triggers and improved data representation through compression and calculation of high-level quantities. These tasks must be performed with low-latency (i.e. in real-time) and often in extreme environments including high radiation, high magnetic fields, and cryogenic temperatures.

==> Instrumentation/Instrumentation.tex <==

\setcounter{chapter}{7} 

\chapter{Instrumentation Frontier}

\authorlist{P. Barbeau, P. Merkel, J. Zhang}
   {D.~Acosta, T.~Affolder, A. Apresyan, G. Carini, T.~Cecil, A.~Connolly, C.E.~Dahl, A.~Deiana, C. O.~Escobar, J.~Estrada, 
J.~Fast, R.~Guenette,
K.~Irwin, A.~Karle, W.~Ketchum,  R.~Maruyama,  M.~Garcia-Sciveres, M.~Newcomer, J. Parsons, 
M.~Pyle, J.~Raaf, C.~Rogan, I.~Shipsey, B.~Surrow, M.~Titov, S.~Vahsen, A.~White, S.~Worm, M.~Yeh, 
R.~Yohay}
\begin{center}
    {\footnotesize M.~Artuso, V.~Bhopatkar, S.~Butalla, K.~Dunne, F.~Fahim, M.~Hedges, S.~Kravitz, H.~Lippincott, J.~McIver, M.~Sanchez, C.~Vernieri, J.~Zettlemoyer}
\end{center}

\section{Executive Summary}
Detector instrumentation is at the heart of scientific discoveries. Cutting edge technologies enable US particle physics to play a leading role worldwide. This report summarizes the current status of instrumentation for high energy physics, the challenges and needs of future experiments and indicates high priority research areas. We also lay out five high-level key messages that are geared towards ensuring the health and competitiveness of the US detector instrumentation community, and thus the entire particle physics landscape. The Instrumentation Frontier studies detector technologies and R\&D needed for future experiments in collider physics, neutrino physics, rare and precision physics and at the cosmic frontier. It is divided into more or less diagonal areas with some overlap among a few of them. 

For the field of high energy physics to continue to have a bright future, priority within the field must be given to investments in both evolutionary and transformational detector development that is coordinated across the national laboratories and with the university community, international partners, other disciplines and industry. While the fundamental science questions addressed by high energy physics have never been more compelling, there is acute awareness of the challenging budgetary and technical constraints when scaling current technologies. Furthermore, many technologies are reaching their sensitivity limit and new approaches need to be developed to overcome the currently irreducible technological challenges. This situation is unfolding against a backdrop of declining funding for instrumentation, both at the national laboratories and in particular at the universities. This trend has to be reversed for the country to continue to play a leadership role in particle physics. In this challenging environment it is essential that the community invest anew in instrumentation and optimize the use of the available resources to develop new innovative, cost-effective instrumentation. We need to invest in modernized facilities with enhanced capabilities, address intermediate planned project needs, and carry out blue-sky R\&D that enable new physics opportunities to successfully accomplish the mission of high energy physics. 

Much of the HEP portfolio is dominated by mid-sized to large scale experiments, which take decades to design, build and operate, and often span the entire lifetime of individuals' careers. In this environment it is becoming increasingly difficult for students and young researchers to have the opportunity to learn hands-on about detector instrumentation. For example on the collider physics side, there will be potentially a large gap in time between the current HL-LHC upgrades finishing and concrete designs and construction for the next generation collider experiments starting. The key challenge here will be to maintain the technical skills and experience within the community, and to train a new generation of instrumentation experts. This gap will have to be bridged partially by an increased effort in generic detector R\&D, as well by encouraging and supporting PIs to get involved in other short-term, smaller scale experiments in other areas, such as astro-particle physics or accelerator-based dark matter and rare processes experiments. An expansion into newly enabled QIS experiments, exploiting recent transformative technological advances should also be encouraged. In general, careers in detector instrumentation in HEP need better support. A valuable addition would be increased opportunities for interdisciplinary PhDs, leveraging the SCGSR program. 
%Students must be able to get a PhD in instrumentation alone, which will be valued at the same level as %those that also led to physics publications. 
Furthermore, the field needs more mid-career positions for instrumentation experts, especially at Universities, where an additional advantage lies in the potential for cross-cutting positions with other departments, such as material science, quantum information, or engineering disciplines.

In addition to the maintenance of the technical workforce and expertise, it is also crucial that the community invests in modern facilities, which enable breakthrough advances in detector technologies for future experiments. A coherent set of supporting facilities needs to be maintained and enhanced over the coming years. Furthermore, the US HEP community needs to consider the creation of a detector R\&D collaborative framework similar to the current RD collaboration model at CERN. These could be in specific technological areas and under the guidance and oversight of CPAD. 

In order to stimulate transformational breakthroughs, we need to pursue synergies with other disciplines  outside of HEP, as well as close collaborations with industry. Recent successful examples of this are QIS and Microelectronics, where communication and exchange between the HEP and other communities led to enhanced funding for technology development, which together with a new suite of available or achievable detector technologies and methods opened up a new suite of small-scale experiments that enhance the HEP portfolio, and can in turn contribute new solutions to traditional experiments. 

To conclude, the science frontiers, CF, EF, NF and RPF, are pursuing a breadth of different future experiments, which have aggressive schedules and are technically challenging. They urgently require significant developments within the instrumentation frontier, which in turn requires significant investment now. The key challenges can be summarized as follows:
\begin{itemize}
    \item[\bf IF-1] {Advance performance limits of existing technologies and push new techniques and materials, nurture enabling technologies for new physics, and scale new sensors and readout electronics to large, integrated systems using co-design methods.}
    \item[\bf IF-2] {Develop and maintain the critical and diverse technical workforce, and enable careers for technicians, engineers and scientists across disciplines working in HEP instrumentation, at laboratories and universities.}
    \item[\bf IF-3] {Double the US Detector R\&D budget over the next five years, and modify existing funding models to enable R\&D Consortia along critical key technologies for the planned long term science projects, sustaining the support for such collaborations for the needed duration and scale.}
    \item[\bf IF-4] {Expand and sustain support for blue-sky, table-top R\&D, and seed funding. Establish a separate review process for such pathfinder R\&D.}
    \item[\bf IF-5] {Develop and maintain critical facilities, centers and capabilities for the sharing of common knowledge and tools, as well as develop and maintain close connections with international technology roadmaps, other disciplines and industry.}
\end{itemize}


\section{Key Technology Needs and R\&D}
\subsection{Quantum sensors}
The use of quantum sensors in high energy physics has seen explosive growth since the previous Snowmass Community Study. This growth extends far beyond high energy physics (HEP) impacting many areas of science from communications to cryptography to computing.  Quantum sensors have been used in searches for dark matter - particle and wave, fifth forces, dark photons, permanent electric dipole moment (EDM), variations in fundamental constants, and gravitational waves, among others. These sensors come in a wide range of technologies: atom interferometers and atomic clocks, magnetometers, quantum calorimeters and superconducting sensors to name a few. Early work with quantum sensors in the context of particle physics often focused in cosmic and rare and precision frontiers, but recent concepts seek to expand the use of quantum sensors to the energy and neutrino frontiers solidifying them as fundamental technologies for the future of experimental HEP. Based upon input to the Snowmass process and outlined in our topical group report~\cite{Cecil2022},  our topical group has identified several key messages necessary to support the development and use of quantum sensors in HEP:

 \begin{itemize}
    \item[\bf IF01-1] \textbf{Continue strong support for a broad range of quantum sensors. Quantum sensors address scientific needs across several frontiers and different technologies carve out unique parameter spaces.} While these sensors share many common characteristics, each has advantages that make it the sensor of choice for specific applications along with challenges that need further development to make the greatest impact.  
    \item[\bf IF01-2] \textbf{Continue support for R\&D and operation of table-top scale experiments. Many are shovel ready and have the potential for large impact.} Much of the growth in quantum sensors over the past decade has occurred in small, laboratory based experiments. 
    These fast-paced small experiments should continue to be supported as a way to rapidly develop sensor technology and help determine those areas where quantum sensors can have the greatest impact.
    \item[\bf IF01-3] \textbf{Balance support of tabletop experiments with pathfinders R\&D to address the large-scale challenges of scaling up experiments which will require National Lab and HEP core competences.} As the fast-paced, small experiments mature, those with significant discovery potential begin to emerge along with areas of commonality between the experiments (e.g.\ the need for advanced high field magnets for axion dark matter experiments or ultra-stable lasers for atom interferometers and clocks). They have reached the point at which plans for larger-scale, longer-term experiments should be conceptualized. These concepts can evaluate the potential reach that can be achieved in a larger effort and the scale of require technological development. 
    \item[\bf IF01-4]  \textbf{Develop mechanisms to support interactions outside of the HEP program to enable collaborations with fields with developed expertise in quantum sensors. Advances in quantum information science (QIS) provide exceptional theoretical and experimental resources to advance quantum sensing that could provide mutual benefits in several areas such as materials, detectors, and devices.} Many of the most promising quantum sensors for HEP science have been developing for the past decade or more in areas outside of the traditional HEP science and funding sphere. For example, atomic clocks developed over many decades as a source of precision timing standards are now stable enough they can be used in the search for variations of fundamental constants and gravitational waves. The HEP community should strive to collaborate with these broader communities in a way the gives HEP access to new sensor technologies while sharing HEP expertise (e.g.\ large magnets and vacuum systems). Effort should be made to allow the free flow of ideas and effort across traditional funding boundaries to encourage scientists and engineers working with quantum sensors to tackle the most interesting and challenging problems available. 
    \item[\bf IF01-5] \textbf{Develop mechanisms to facilitate interactions to support theoretical work address issues of materials and measurement methods.} As with other instrumentation frontiers and as quantum sensors become more sensitive, focused support on quantum materials at the interface of quantum sensors and HEP will be needed. This includes theoretical work necessary for on topics including quantum materials, squeezing, and back action.
    \item[\bf IF01-6] \textbf{Workforce development is needed to encourage workers with the needed skills to engage with the HEP field, maintain current momentum, and for long-term success in the face of growing competition from industrial quantum computing.} While the high energy physics community is poised to benefit from quantum sensor developments outside of HEP, we face a shortage of skilled workers. The explosive growth in quantum computing in recent years, along with arrival of several major tech companies has created a fierce competition for workers with skills needed to develop quantum sensors and experiments. The HEP community will need to invest now in order to train and retain the next generation of quantum scientist. Increasing collaborations outside of HEP -- as discussed above -- can provide an additional pathway to reaching skilled workers and engaging them on HEP challenges.  
\end{itemize}

\subsection{Photon Detectors}

The Photon Detectors Topical Group has identified two areas where focused R\&D over the next decade could have a large impact in High Energy Physics Experiments. These areas described here are characterized by the convergence of a compelling scientific need and recent technological advances. A short summary can be found below, while a more extensive report, including a large number of references for further reading, is given in the Photon Detector Topical Group report~\cite{IF02-report}.

The development of detectors with the capability of counting single photons from IR to UV has been a very active area in the last decade. Demonstration for sensors based on novel semiconductor (CMOS, skipper-CCD, SiPM) and superconducting technologies (MKID, SNSPD and TES) have been performed. These sensors open a new window for HEP experiments in the low photon number regime. Several ongoing and future projects in HEP benefit from these developments (Cosmology, Dark Matter, Neutrinos) which will also have a large impact outside HEP (BES, QIS, Astronomy). The combined scientific needs and technological opportunities make photon counting an ideal area for focused R\&D investment in the coming decade.  R\&D is needed for enabling large arrays of the new sensors, improving their energy resolution, timing, dark counts rates and extending their wavelength coverage. Such investment will secure leadership in photon counting technologies in the US, producing a large impact in HEP, with applications outside HEP. This opportunity is summarized in Ref~\cite{PhotonCountingWP}.

A technological solution for the photon detection system in the first two modules of the
DUNE detector exist, based on the by now well-known Arapuca light traps, with wavelength shifters and SiPMs as the photon detector. However, new photon detector developments are being considered
for modules 3 and 4. Some of the proposed ideas consist on novel light collectors, the so-called dichroicons which are Winston-style light concentrators made from dichroic mirrors,
allowing photons to be sorted by wavelength, directing the long-wavelength end of broad-band Cherenkov
light to photon sensors that have good sensitivity to those wavelengths, while directing narrow-band shortwavelength
scintillation light to other sensors. This technology could be used in water-based liquid scintillators thus realizing a hybrid Cerenkov and scintillator detector. 

One significant development in the last decade is the commercialization of Large Area Picosecond Photodetectors (LAPPDs) and their 
first deployment in a neutrino experiment (ANNIE). LAPPDs are imaging single-photon sensors, capable of resolving photon hit positions with sub-cm resolution and arrival times of around 50 ps. LAPPDs bring capabilities that may make them useful in future LAr detectors, and as part of the DUNE near detector system, particularly ND-GAr. They also have the requisite time resolution to separate between early-arriving Cherenkov light and slower scintillation light.

Also notable are research and development efforts in new materials that could be directly sensitive to the VUV light, such as amorphous selenium (a-Se) and organic semiconductors. R\&D is needed to move from concept demonstrations to full scale implementations in an HEP experiment. Future investment in the above technologies over the next decade will enhance the science 
of the DUNE project.

The science for generation, detection and manipulation of light is extremely fast moving and driven mainly from outside our field. The HEP community would benefit from resources dedicated to the implementation of these advanced photonic technologies in particle physics experiments. 

\begin{itemize}
\item[\bf IF02-1]  The development of detectors with the capability of counting single photons from IR to UV has been a very active 
area in the last decade. We now need to pursue R\&D to 
implement these in HEP experiments by making larger arrays,
improving their energy resolution, timing, dark counts rates and extending their wavelength coverage. 

\item[\bf IF02-2]  New photon detector developments are being considered for planned future neutrino experiments going beyond the current technologies. Concept demonstrations have been done, and we now need to move from a conceptual phase to working detectors.
\end{itemize}

\subsubsection{Photon Counting Sensors Enabling HEP}
Several novel cosmological facilities for wide-field multi-object spectroscopy were proposed for the Astro2020 decadal review, and are being considered as part of the Snowmass process. 
Ground-based spectroscopic observations of faint astronomical sources in the low-signal, low-background regime are currently limited by detector readout noise. Significant gains in survey efficiency can be achieved through reductions by using sensors with readout noise below 1e-. Pushing the current photon counters in the direction of mega pixel arrays with fast frame rate (about 10 fps) would make this possible.

Dark matter searches  based on photon counting technologies currently hold the world record sensitivity for low mass electron-recoil dark matter semiconductors are among the most promising detector technologies for the construction of a large multi-kg experiment for probing electron recoils from sub-GeV DM (skipper-CCDs). Significant R\&D is needed to scale to scale the experiments from the relatively small pathfinders to the multi-kg experiments in the future. 

Single photon counting sensors have also gained importance for their potential as CEvNS detectors. (Coherent Elastic neutrino Nucleus Scattering). The deposited energy from CEvNS is less than a few keV. Only part of this energy is converted into detectable signal in the sensor (ionization, phonons, etc.) and therefore low threshold technologies are needed. Semiconductor and superconducting technologies with eV and sub-eV energy resolution for photon counting capability in the visible and near-IR are natural candidates to reach the necessary resolution for this application.

Photon counting also enables a wide range of science outside HEP including QIS, BES and applications in radiation detection.

Recent advances in photon counting technology are discussed here. The advances can be grouped in three areas. 

\paragraph{Superconducting Sensors}
\subparagraph{MKIDs} (microwave kinetic inductance detector) work on the principle that incident photons change the surface impedance of a superconductor through the kinetic inductance effect. The magnitude of the change in surface impedance is proportional to the amount of energy deposited in the superconductor, allowing for single photon spectroscopy on chip. Frequency multiplexed arrays  20,440 pixels with energy resolution R=E/$\Delta$E$\sim$9.5 at 980 nm, and a quantum efficiency of ${\sim}$35\% have been achieved. R\&D focused on larger arrays with higher QE and better energy resolution would address the needs of the community.

\subparagraph{SNSPDs} (Superconducting Nanowire Single Photon Detector) is a superconducting film patterned into a wire with nanometer scale dimensions (although recently devices with micrometer-scale widths have been shown to be single-photon sensitive). SNSPDs have been reported with single photon sensitivity for wavelengths out to several microns, 
timing jitter as low as a few~ps, dark count rates (DCR) down to $6\times10^{-6}$ Hz, and 
detection efficiency (DE) of 0.98. They have also been  have been shown to function in magnetic fields of up to 6T. Current R\&D consist on scaling to large arrays and extending the spectral range for these sensors to address 
the needs of HEP and Astrophysics.

\subparagraph{TES} (Transition-Edge Sensor)  photon detector, which utilizes a patterned superconducting film with a sharp superconducting-to-resistive transition profile as a thermometer, is a thermal detector with a well developed theoretical understanding. 
When a visible or infrared photon is absorbed by a TES, the tiny electromagnetic energy of the photon increases the temperature of the TES and therefore changes its resistance. TES have been developed to measure single photons in quantum communication, for axion-like particle searches, direct detection of dark matter particles and astrophysical observations in the wavelengths between ultraviolet and infrared. TES detectors can be multiplexed enabling arrays of large channel counts. Multiplexers for detector arrays using 16,000 TESs have already been successfully implemented R\&D  exploiting microwave resonance techniques have the potential to increase the multiplexing capacity by another factor of 10. 

\paragraph{Semiconducting Sensors}
\subparagraph{Skipper-CCDs} Skipper-CCDs have an output readout stage that allows multiple non-destructive sampling of the charge packet in each pixel of the array thanks to its floating gate output sense node. This non-destructive readout has been used to achieve deep sub-electron noise in mega-pixel arrays Skipper CCDs fabricated on high resistivity silicon has also demonstrated an extremely low production of dark counts. This technology as motivated to build a new generation of Dark Matter and neutrino experiments. The R\&D effort here is currently is currently focused on faster readout (10 fps) and large gigapixel arrays.

\subparagraph{CMOS} The down scaling of CMOS technology has allowed the implementation of pixels with a very low capacitance, and therefore, high sensitivity and low noise (1-2\,$\rm e^-$) at room temperature and high frame rates (50-100\,fps). Commercial cameras  with  sub-electron noise at 5\,fps are now available. These sensors have not yet played a big role in HEP mainly because of the small pixel size. Active R\&D taking advantage of CMOS fabrication process to address the needs of HEP is ongoing to produce, including the development of new CMOS sensors with non-destructive readout (skipper-CMOS). These sensors could address the readout speed limitations of other semiconductor photon counters. The single photon avalanche diode (SPADs) have also been implemented in standard CMOS technology and integrated with on-chip quenching and recharge circuitry addressing fast timing and radiation tolerance requirements from HEP.

\subparagraph{Photon-to-Digital converter} In a PDC, each SPAD is coupled to its own electronic quenching circuit.
This one-to-one coupling provides control on individual SPADs and signals each detected avalanche as a digital signal to a signal processing unit within the PDC. Hence, PDCs provide a direct photon to digital conversion considering that intrinsically a SPAD is a Boolean detector by design. Digital SiPMs were first reported in 1998 by the MIT Lincoln Lab and many contributions followed.
A major step came with microelectronics integration to fabricate both the SPAD and readout quenching circuit in a single commercial process. 
These innovations led to the first multi-pixel digitally read SPAD arrays. A recent review can be found in Ref.~\cite{Pratte2021_Sensors}. 

\paragraph{Extending Wave Length Coverage}
\subparagraph{Ge semiconductor}
Silicon CCDs are commonly utilized for scientific imaging applications in the visible and near infrared. These devices offer numerous advantages described previously, while the skipper CCD adds to these capabilities by enabling multiple samples during readout to reduce read noise to negligible levels. CCDs built on bulk germanium offer all of the advantages of silicon CCDs while covering an even broader spectral range. The R\&D in this area will extend the photon counting capabilities of semiconductor into the IR.

\subparagraph{UV}
It has been shown that CCD sensitivity can be increased close to the reflection-limited quantum efficiency of silicon.
This was done by blocking the surface fields and traps through the epitaxial growth of a strongly doped very thin silicon layer (delta-doping).
Quantum efficiency exceeding 50\% was demonstrated in CCDs down to 125~nm wavelength.
The method was demonstrated efficiently on backside-illuminated SPAD-based detectors.
Other methods to address the surface field and trap issues were also demonstrated.
Work is being done to enhance SiPMs for the detection of the fast scintillation component of BaF$_2$.
An extensive study of the delta-doping approach to enhance VUV sensitivity in frontside-illuminated SPAD-based detectors has also been carried out.

\subsubsection{Photon Detectors For Neutrino Experiments}
A large number of outstanding questions remain to the fundamental nature of the neutrino, which can be probed through the use of higher energy ($\mathcal{O}$(MeV) $< E < \mathcal{O}$(GeV)) neutrino sources (\eg, accelerator and atmospheric neutrinos). The nature of these remaining puzzles break into the distance over which the neutrinos are allowed to propagate before being detected. Thus the future class of experiments are classified as ``short-baseline'' and ``long-baseline'' experiments. 

The next generation long-baseline neutrino experiments aim to answer the questions of the exact ordering of the neutrino mass states, known as the mass hierarchy, as well as the size of the CP-violating phase $\delta$. These, as yet unknown quantities, remain one of the last major pieces of the Standard Model of particle physics and offer the opportunity to answer such fundamental questions as ``what is the origin of the matter/antimatter asymmetry in the universe?'' and ``do we understand the fundamental symmetries of the universe?''. By measuring the asymmetry between appearance of electron neutrinos from a beam of muon neutrinos ($P(\nu_{\mu} \rightarrow \nu_{e}$)) compared to the appearance of electron antineutrinos from a beam of muon antineutrinos and $P(\bar{\nu}_{\mu} \rightarrow \bar{\nu}_{e}$)) as well as the precise measurement of the $\nu_{e}$ energy spectrum measured at the far detector, both the CP violating phase ($\delta_{CP}$) and the mass hierarchy can be measured in the same experiment.

The Short-Baseline Neutrino (SBN) program aims to address the anomalous neutrino results seen by the LSND and MiniBooNE which suggest the possible existence of a eV mass-scale sterile neutrino. However, the experimental landscape is perplexing since a number of other experiments utilizing a range of different neutrino sources which should have been sensitive to such a sterile neutrino have observed only the standard three neutrino oscillations. In this landscape, the conclusive assessment of the experimental hints of sterile neutrinos becomes a very high priority for the field of neutrino physics.

To address both of these areas of neutrino research, large scale noble element time projection chambers (TPC's) play a central role and offer an opportunity to perform discovery level measurements through the enhancement of their capabilities. In a noble element TPC, particles interact with the medium and deposit their energy into three main channels: heat, ionization, and scintillation light. Depending on the physics of interest, noble element detectors attempt to exploit one or more of these signal components. Liquid Noble TPC's produce ionization electrons and scintillation photons as charged particles traverse the bulk material. An external electric field allows the ionization electrons to drift towards the anode of the detector and be collected on charge sensitive readout or transform energy carried by the charge into a secondary pulse of scintillation light. 

A technological solution for the photon detection system in the first two modules of the
DUNE detector exist, based on the by now well-known Arapuca light traps, with wavelength shifters and SiPMs as the photon detector. This approach 
is also being used in other short baseline neutrino oscillation experiments, but not exclusively. Beyond this,new photon detector developments 
are being considered for modules 3 and 4 as well as for other approved or proposed experiments. 

\paragraph{Going beyond DUNE's first two modules}: 
Quoting from the executive summary of the Snowmass IF2 White Paper\emph{Future Advances in Photon-Based Neutrino Detectors}~\cite{Klein},
"large-scale, monolithic detectors that use either Cherenkov or scintillation light have played major roles in nearly every discovery of neutrino oscillation phenomena or observation of
astrophysical neutrinos. New detectors at even larger scales are being built right now, including JUNO,
Hyper-Kamiokande, and DUNE.

These new technologies will lead to neutrino physics and astrophysics programs of
great breadth: from high-precision accelerator neutrino oscillation measurements, to detection of reactor and solar
neutrinos, and even to neutrinoless double beta decay measurements that will probe the normal hierarchy regime.
They will also be valuable for neutrino applications, such as non-proliferation via reactor monitoring".

"Of particular community interest is the development of hybrid Cherenkov/scintillation detectors, which can simultaneously
exploit the advantages of Cherenkov light|reconstruction of direction and related high-energy particle identification (PID)
and the advantages of scintillation light, high light-yield, low-threshold detection with low-energy PID. Hybrid
Cherenkov/scintillation detectors could have an exceptionally broad dynamic range in a single experiment, allowing
them to have both high-energy, accelerator-based sensitivity while also achieving a broad low-energy neutrino
physics and astrophysics program. Recently the Borexino Collaboration has published results showing that even in a detector with standard scintillator and no special photon sensing or collecting, Cherenkov and scintillation light can be discriminated well enough on a statistical basis that a sub-MeV solar neutrino direction peak can be seen. Thus the era of hybrid detectors has begun, and many of the enabling technologies described here will make full
event-by-event direction reconstruction in such detectors possible".

Among the new technologies of relevance for this topical group, it should be mentioned 
\paragraph{Large Area Picosecond Photodetectors}: New advances in the science of photomultiplier tubes, including long-wavelength
sensitivity, and significant improvements in timing even with devices as large as 8 inches, make hybrid
Cherenkov/scintillation detectors even better, with high light yields for both Cherenkov and scintillation light
with good separation between the two types of light. Large Area Picosecond Photon
Detectors (LAPPDs) have pushed photon timing into the picosecond regime, allowing Cherenkov/scintillation
separation to be done even with standard scintillation time profiles. The fast timing of LAPPDs also makes
reconstruction of event detailed enough to track particles with the produced photons.
The precision timing capabilities of LAPPDs make possible new stroboscopic techniques where different energy components of a wide-band neutrino beam can be selected based on the arrival of the neutrinos relative to the beam RF timing. Future neutrino experiments, including possible upgrades to LBNF, could enable sufficiently short proton bunches to make this technique viable. At the detector end, this technique requires time resolutions on the order of no more than a few hundred picoseconds. Hybrid Cherenkov-scintillation detectors with LAPPDs are naturally well suited for this level of vertex precision.

The continued use and development of application readiness of LAPPDs in experiments like ANNIE is critical to their future viability. Additional investments in R&D to further grow production yields and reduce costs will also benefit future large-scale HEP efforts. 
\paragraph{Dichroicons}: Dichroicons, which are Winston-style light concentrators made from dichroic mirrors,
allow photons to be sorted by wavelength thus directing the long-wavelength end of broad-band Cherenkov
light to photon sensors that have good sensitivity to those wavelengths, while directing narrow-band shortwavelength
scintillation light to other sensors. Dichroicons are particularly useful in high-coverage hybrid
Cherenkov/scintillation detectors. 

\subsection{Solid State Detectors and Tracking}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

Tracking detectors are of vital importance for collider-based high energy physics (HEP) experiments. The primary purpose of tracking detectors is the precise reconstruction of charged particle trajectories and the reconstruction of secondary vertices. The performance requirements from the community posed by the future collider experiments require an evolution of tracking systems, necessitating the development of new techniques, materials and technologies in order to fully exploit their physics potential. 

%Relative to the currently operating systems and their upgrades, the technical requirements for tracking detectors (trackers) in the next 20-40 years are significantly more stringent, such as tolerances to fluences 1-2 orders of magnitude higher, larger areas at lower costs, segmentation and position resolution 2-4 times finer and precision timing resolution, radiation length per layer from 0.1-1\% $\rm{X_{0}}$ and integration of novel radiation-hard materials. 

%\begin{itemize}
%    \item Tolerance to fluences 1-2 orders of magnitude higher
%    \item Larger areas at lower costs 
%    \item Segmentation and position resolution 2-4 times finer
%    \item Precision timing resolution in a tracking environment
%    \item Radiation length per layer from 0.1-1\% $\rm{X_{0}}$
%    \item Cooling below the triple-point of $\rm{CO_{2}}$
%    \item Integration of novel radiation-hard materials
%\end{itemize}

Technological developments currently underway aim to address these issues, and the successful completion of the programs outlined below 
%will be a important step towards the delivery of tracking detectors meeting these goals. 
%Successful completion of these programs 
%% what programs?
requires focused efforts from the community on the steady development and refinement of existing technologies, and the pursuit of novel 
``blue sky'' technologies to enable transformative progress. The HEP community gathered at Seattle Snowmass Summer Meeting in 2022 identified the following key directions for the near-term priorities of the solid-state tracking:

\begin{itemize}
    \item \textbf{IF03-1}: Develop high spatial resolution pixel detectors with precise per-pixel time resolution to resolve individual interactions in high-collision-density environments
    \item \textbf{IF03-2}: Adapt new materials and fabrication/integration techniques for particle tracking in harsh environments, including sensors, support structures and cooling
    \item \textbf{IF03-3}: Realize scalable, irreducible-mass trackers in extreme conditions
    \item \textbf{IF03-4}: Progress advanced modeling for simulation tools, developing required extensions for new devices, to drive device design.  
    \item \textbf{IF03-5}: Provide training and workforce maintenance to enable future tracking systems to be designed, developed, constructed and simulated.
    \item \textbf{IF03-6}: Nurture collaborative networks, provide technology benchmarks and roadmaps and funding in order to develop required technologies on necessary time scales, costs and scope.
\end{itemize}

%Eight white papers on solid state trackers were submitted during the 2022 Snowmass~\cite{arxiv.2202.11828,arxiv.2203.06093,arxiv.2203.06773,arxiv.2203.07626,arxiv.2203.08554,arxiv.2203.13900,arxiv.2203.06216,arxiv.2203.14347}, focusing on a broad set of R\&D topics that the US community is actively pursuing. While these papers don't completely capture the full breadth and depth of the R\&D carried out in the US, they highlight the key challenges that future trackers will face and summarize the main research thrusts actively pursued by the community. 

%Such issues has been foreseen by technological developments currently underway; successfully completion of these programs should enable the delivery of trackers meeting these goals.  

%At a future 100 TeV p-p hadron collider, for example, one of the primary challenges will be the efficient reconstruction of charged particle tracks in an environment of unprecedented pileup density. An integrated 4-dimensional tracker with hit timing resolution at the levels of $\sim$10~ps will drastically reduce the combinatorial challenge of track reconstruction at extremely high pileup densities. Trackers with precise timing and directional information at a muon collider will allow to not only handle the beam-induced-backgrounds, but will also enable the experiments to take high quality data for precision measurements and searches for new physics at highest energies. At $e^+e^-$ or electron-ion colliders the use of 4D trackers is primarily focused on particle identification and vertex identification. Additionally, timing information offers completely new handles to detect and trigger on long-lived particles (LLP) [2,4], expand the reach to search for new phenomena [2], and enable particle-ID capabilities for pion/kaon separation at low transverse momentum [2]. 4D devices with coarse timing capabilities at $\sim$ns level but with similar granularity as regular tracking devices at the other end of 4D phase space can complement the fast timing layers for an enhanced overall 4D tracking.

Advanced 4-dimensional trackers with ultra fast timing (10-30~ps) and extreme spatial resolution (O(few~$\mu$m)) represent a new avenue in the development of silicon trackers, enabling a variety of physics studies which would remain out of experimental reach with the existing technologies. Several technology solutions are being currently pursued by the community to address the challenges posed by various experiments~\cite{arxiv.2203.13900,arxiv.2203.06773,arxiv.2203.08554}, both for the sensors~\cite{arxiv.2202.11828} and the associated electronics. The packaging and integration of the sensors and readout electronics will become more critical for future experiments, as device segmentation decreases to mitigate the increased track density. Bump bonding technologies have nearly reached their limits; more advanced 3D packing technologies including wafer-to-wafer and die-to-wafer hybrid bonding and through silicon vias (TSV) have the potential to meet the goals of future particle physics experiments~\cite{arxiv.2203.06093,arxiv.2203.07626}.  

Detector mechanics will also play a significant role in future detectors' performance.  Material necessary for cooling and structural stability will be the lower bound on the radiation length for future tracking systems. Increased segmentation will lead naturally to larger power densities; in order to minimize material, solutions with integrated services and cooling are necessary. A holistic approach to design, simulation and manufacturing will be required. Novel materials, new cooling and composite manufacturing technique will need to be developed in order to reach the targeted performance~\cite{arxiv.2203.14347}. 

To develop these new technologies, simulations of the properties of silicon and novel sensor materials throughout the lifetime of the experiments will be critical.  These studies can drive device design included implant locations, size and strength to the most promising directions of development~\cite{arxiv.2203.06216}. To reach their full potential, further developments are needed to improve accuracy, precision and new devices.   With this research, the performance of future experiments can be better predicted for its full life cycle prior to construction.  

\subsection{Simulations of Silicon Radiation Detectors for High Energy Physics Experiments}

There are currently a variety of  tools available for simulating the properties of silicon sensors before and after irradiation.  These tools include finite element methods for device properties, dedicated annealing models, and testbeam/full detector system models.  No one model can describe all of the necessary physics.  Most of these models are either fully or partially developed by HEP scientists and while there are many open-source tools, the most precise device property simulations rely on expensive, proprietary software. 

While existing approaches are able to describe many aspects of signal formation in silicon devices, even after irradiation and annealing, there is significant R\&D required to improve the accuracy and precision of these models and to be able to handle new devices (e.g. for timing) and the extreme fluences of future colliders.  The US particle physics community can play a key role in this critical R\&D program, but it will require resources for training, software, testbeam, and personnel. 

For example, there is a great need for (1) a unified microscopic model of sensor charge collection, radiation damage, and annealing (no model can currently do all three), (2) radiation damage models (for leakage current, depletion voltage, charge collection) with uncertainties (and a database of such models), and (3) a measurement program to determine damage factors and uncertainties for particle types and energies relevant for current and future colliders. Equipped with these tools, the US community can play a key role in the success of future collider physics, and help in defining the most promising avenues to realize the necessary performance of future experiments. 

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Novel Sensors for Particle Tracking}

The proposed future collider experiments pose unprecedented challenges for event reconstruction, which require development of new approaches in detector designs. Several technologies are currently being investigated to develop technologies for the future, which approach these goals in complementary ways. 

Silicon or diamond sensors with ``3D technology" have electrodes oriented perpendicular to the plane of the sensor. New 3D geometries involving p-type trench electrodes spanning the entire thickness of the detector, separated by lines of segmented n-type electrodes for readout, promise improved uniformity, timing resolution, and radiation resistance. Present research aims for operation with adequate signal-to-noise ratio at fluences approaching $10^{18}~n_{\rm eq}/{\rm cm}^2$, with timing resolution on the order of 10 ps. 

Monolithic Active Pixel Sensors (MAPS), in which charge collection and readout circuitry are combined in the same pixel, have been shown to be a promising technology for high-granularity and low material budget detector systems. MAPS have several advantages over traditional hybrid pixel detector technologies, as they can be inexpensively fabricated in standard CMOS imaging processes, back-thinned or back-illuminated, have demonstrated high radiation hardness. Many MAPS pixel geometries have been explored, but the close connection of a sensor and front-end amplifier, without the need for external interconnections, holds the promise of reducing the input capacitance significantly, and hence extremely low-noise designs are possible. The reduction of the noise floor means that even small signals, for example from thinned low-power sensors, can yield satisfactorily high S/N. 

Thin film detectors  have the potential to be fully integrated, while achieving large area coverage and low power consumption with low dead material and low cost.  Thin flim transistor technology uses crystalline growth techniques to layer materials, such that monolithic detectors may be fabricated by combining layers of thin film detection material with layers of amplification electronics using vertical integration.

\subsection{4-Dimensional trackers}
\label{sec:if03_4Dtrackers}

Future collider experiments call for development of tracking detectops with 10-30~ps timing resolution, in addition to excellent position resolution, i.e. 4-Dimensional trackers. Time resolution of the future 4D tracker detector can be factorized into contributions from the sensor itself, and those from the readout electronics. The overall detector system should contain a sensor with short drift time, high signal to noise, limited thickness in the path of a MIP to reduce the Landau fluctuations, and small TDC bin size. Several technologies to address these needs are being developed and are introduced in this section. 

Several modifications to Low Gain Avalanche Detectors (LGADs) technology have been proposed and demonstrated to make them suitable for tracking sensors with 100\% fill-factor, achieving excellent timing and position resolution. A key feature of AC-LGADs is the signal sharing between electrodes, which can be used to obtain the  simultaneous 30~ps and 5~$\mu$m resolutions. Another design geared towards 100\% fill factor are the ``Deep-Junction'' (DJ-LGAD), which are formed by abutting thin, highly-doped p$+$ and n$+$ layers. `Buried Layer LGADs'' aim to achieve higher radiation tolerance by implanting the boron layer at low energy, and then burying it under a few microns of epitaxially grown silicon. 

Another thrust to develop 4D-tracking sensors is through a usage of novel sensors with 3D geometries, or closer integration with electronics via monolithic pixel sensors, or adoption of new materials in sensor design. Going even beyond 4D-sensors are designs that aim to simultaneously measure not only the position and time, but also the angle of passing tracks. These kind of sensors would dramatically reduce the complexity of detector modules, and enable unprecedented reconstruction capabilities on the front-end. Double Sided LGADs (DS-LGADs) achieve this goals by adding a readout layer to the p-side of the LGAD structure, which allows one to also measure signals from the slower-drifting holes.

The timing ASICs under development for the ATLAS and CMS timing upgrades, named ALTIROC and ETROC, represent revolutionary steps forward as the first readout chips to bring O(10~ps) timing to collider experiments. However, they are able to use significantly more space and power than high density ASICs designed for trackers with fine pitch and limited material. Compared to RD53A, the timing chips use several hundred times more power and area per channel. The primary challenges to transform them into chips for 4D tracking will be to minimize both the power consumption and the channel size. Currently there are  several projects with the aim to make advance in these areas, more details are listed in Sec. ~\ref{sec: sec:if03_4Dtrackers}. 

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Integration}

In the past years, HEP experiments have been mostly relying on bump bonding for high density pixel sensor to ASIC connection. 
The bump bonding technology was proven to be reliable; however, it is known to have several limitations: it only works down to 20-50~$\mu m$ of pitch and has yield issues for finer connections. 
Furthermore, the solder balls used for the connection increase the input capacitance to the amplifier and hence the noise. 
With bump bonding,the sensor or chip need side extensions to have external connections.
In terms of mechanical properties the resulting connection is subject to heat stress since it involves different materials; the minimum thickness is also limited since both chip and sensor need a thick enough support wafers in order to meet alignment and bow requirements for the bump bonding process. 

The introduction of more advanced packaging can solve many of these issues, allowing for the improvement of performance, yield and processing.
3D integration is a common widespread technology in industry, it allows tight packaging of sensor and readout chip. Furthermore it allows to stacks multiple chips in a single monolithic device. 
There are many technologies available for 3D integration, hybrid bonding is the most widely accepted.
Through Silicon Vias (TSVs) allow multiple planes to be stacked and connected with external connections without the need of extensions or silicon interposers.

Advanced packaging and wafer to wafer bonding would facilitate several applications both in HEP and outside of HEP. 
Therefore electronics and sensor advanced packaging provide a variety of technologies that can meet the needs of future particle physics experiments. 
Combining these capabilities with silicon technologies developed for HEP, such as LGADs and active edge sensors, will allow the design of sophisticated detector systems that can meet the increasing challenges of next generation experiments. 
The collaboration between research groups and industry with established expertise in advanced packaging is crucial for the successful introduction of this technology in the research community. 

Current availability of such technologies is mixed.  Leading edge foundries and nodes now include 3D processes (Intel Forveros, TSMC 3DFabric, Samsung x-cube) but are typically too expensive for HEP. Hybrid bonding is available from many vendors that already work with HEP.  The availability of TSVs is more limited. Small pitch TSVs are available from some foundries at advanced nodes ($>$32 nm), in Silicon-on-Insulator (SOI) wafers, and from specialty foundries.  Larger pitch TSVs inserted in a completed wafer (via-last) are available from a variety of packaging suppliers.  Reliable 3D devices with these large pitch ($>$20 $\mu m$) external TSV connections can be accessed now with resources available to HEP.  It is important to build design and fabrication experience with moderate scale companies now gearing up to address opportunities afforded by the US semiconductor initiative. 

\subsection{Mechanics}
%Contributions for this section from \cite{MechanicsWP}

Detector mechanics will play a significant role in future detectors' performance; the necessary improvements will require simulations, novel ways to reduce the total mass, as well as more integrated design concepts to save on material budgets and optimize performance. The increased segmentation has naturally lead to larger power densities requiring high performance material support structures with integrated services.  In many cases, the material in these structures can be the limiting factor for the tracking performance of the system.  Particle detectors at future colliders rely on ever more precise charged particle tracking devices, which are supported by structures manufactured from composite materials. Various engineering techniques able to solve challenges related to the design and manufacturing of future support structures have been developed.

Future particle colliders, such as the high luminosity Large Hadron Collider (HL-LHC), the Future Circular Collider (FCC-ee, FCC-hh), or the muon collider (MuC) will collide particles at unprecedented rates and present a harsh environment for future detectors. A holistic approach to the design and manufacturing of detector support structures will be necessary to achieve minimal weight systems. Novel techniques, materials and other design and manufacturing solutions provide an avenue to solve challenges of increasingly more complex and large tracking detectors. Complex stresses in composite structures pose a severe challenge to current simulation tools. Research and development efforts are underway to solve these challenges by exploring multi-functional composite structures

Material savings due to novel approaches have the potential of reduction on the order of 30-50\% depending on more detailed R\&D studies. This is an ideal opportunity to explore the conjunction of latest techniques in composite engineering involving machine learning based algorithms for heat transfer, mechanical loading and micro-to-macro scale material response predictions. Different structures are being studied to achieve these goals which include: carbon fiber support structures with integrated titanium pipes for $\rm{CO_2}$ cooling, etched silicon and peak cooling micro-channels, Kapton-based support structures and engineered air cooling. 

\subsection{Collaborative development programs}

Collaborative efforts should be encouraged when possible to make efficient use of resources and reduce the financial burden on individual groups, and to enlarge the pool of expertise in the field. Especially critical is to encourage and support young researchers to engage and pursue intensive research programs to develop these new technologies, which will help to ensure an expert workforce is sustained for the long term. Considering the prohibitively high costs for productions of new technologies at commercial foundries, collaborative submissions can provide the only viable solution for research groups to access advanced production facilities. Such collaborations promise to significantly expand the possibilities for small experiments or small groups to join advanced detector R\&D programs, work with others in the field to build technology demonstrators, and help advance the solid-state tracking technology. 








%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Trigger and DAQ}
A trend for future high energy physics experiments is an increase in the data bandwidth produced from the detectors. Datasets of the Petabyte scale have already become the norm, and the requirements of future experiments---greater in size, exposure, and complexity---will further push the limits of data acquisition technologies to data rates of exabytes per seconds. The challenge for these future data-intensive physics facilities lies in the reduction of the flow of data through a combination of sophisticated event selection in the form of high-performance triggers and improved data representation through compression and calculation of high-level quantities. These tasks must be performed with low-latency (\textit{i.e.} in real-time) and often in extreme environments including high radiation, high magnetic fields, and cryogenic temperatures.

Developing the trigger and data acquisition (TDAQ) systems needed by future experiments will rely on innovations in key areas:
\begin{itemize}
\item[\bf IF04-1] Pursue innovations in the application of Machine Learning (ML) to TDAQ systems, particularly in the co-design of hardware and software to apply ML algorithms to real-time hardware and in other novel uses to improve the operational efficiency and sensitivity to new physics of future experiments;
\item[\bf IF04-2] Invest in the design of TDAQ system architectures that leverage new technologies, techniques, and partnerships to enable more intelligent aggregation, reduction, and streaming of data from detectors to higher-level trigger systems and offline data processing; and, 
\item[\bf IF04-3] Develop improved readout technologies that increase data bandwidth and are capable of operating in extreme environments, while fitting the material and power constraints of future experiments.
\end{itemize} 

Critically, innovations in TDAQ rely on the people and processes behind them, and require investments in those people and infrastructure for R\&D. To that end, we call for:
\begin{itemize}
\item[\bf IF04-4] Increased effort to build and retain domain knowledge for complex TDAQ systems by reliably supporting facilities and people – particularly engineers and technical staff, and early-career scientists through recruitment and training – in order to bring new ideas from early design and prototyping all the way through integration, commissioning, and operation in future detectors; and,
\item[\bf IF04-5] The creation of a dedicated (distributed) R\&D facility that can be used to emulate detectors and TDAQ systems, offer opportunities for integration testing (including low- and high-level triggering, data readout, data aggregation and reduction, networking, and storage), and develop and maintain an accessible knowledge-base that crosses experiment/project boundaries.
\end{itemize}

\subsubsection{A compelling use case: track-based triggers}

Searches for novel new physics are often made possible by the development of novel new triggers that take advantage of improvements in detectors and real-time computing. Early-stage trigger systems of experiments at hadron collider experiments, for example those at the Large Hadron Collider (LHC), often select objects with high momentum, based on calorimeter information, in order to reduce the large backgrounds to events of physical interest.  However, this process necessarily loses many events, and is poorly optimized to explore a variety of potential beyond Standard Model (SM) scenarios.  For instance, low momentum events with displaced vertices could lead to soft-unclustered-energy-patterns, long-lived staus or the decays of long-lived dark scalars in the Higgs portal scenario~\cite{wp_exotracktrig}.  Alternatively, high-momentum and short-lived particles, such as dark matter particulates, might be missed by the existing trigger systems due to their invisible decay within the detector volume~\cite{wp_tracktrig}.

For both of these cases, early-stage triggers based on tracking information could preserve interesting signal events for study.  A difficulty of including tracking information in early-stage triggers is the complexity of calculating tracks and the speed at which decisions need to be made.  For instance, at the LHC~\cite{LHC} events are produced at a rate of 40 MHz, and this must be very rapidly reduced to the kHz level at the first step of the trigger system. The development of a fast track-based trigger is therefore an area of considerable interest in the high energy physics community, and several different approaches have been taken to solve the problem for silicon-strip tracking systems.  
For future hadron collider experiments, a fast tracking trigger for silicon pixel tracking layers at small radii with respect to the beam pipe, and therefore with significantly more channels than strip trackers, would open the sensitivity to particles arising from beyond SM physics in an interesting lifetime regime.

As a new approach, a white paper contributed to
Snowmass~\cite{wp_tracktrig} utilizes highly-parallelized graph
computing architecture using field-programmable gate arrays (FPGAs) to
quickly performing tracking in small-radius silicon detectors.
This paper proposes unsupervised machine learning on a
highly-parallelized graph computer constructed using modern FPGA
technology.
As documented in~\cite{GraphTracking}, this algorithm yields a trigger
efficiency near 100\% for track transverse momenta above 10~GeV and a
spurious trigger rate of a few kHz. Implementation studies on a Virtex
Ultrascale+ FPGA are in progress and indicate a latency of 200~ns,
well below the 4 $\mu$s limit for trigger algorithms at LHC
experiments.

We note that the design of future detector systems, especially tracking systems in dense, high occupancy environments, is best done taking into account the necessary trigger and DAQ considerations early in the process. For example, the design of the HL-LHC silicon tracker for the CMS experiment~\cite{CMSPhase2Tracker} utilizes the local coincidence of hits in two closely-spaced tracking layers to provide some limited momentum selection capability. This is necessary to  reduce the data rate from the detector to manageable levels for the early-level trigger system.  

\subsubsection{Heterogeneous Computing and Machine Learning}

As is well known, the scaling of single CPU solutions to efficiently address computational problems has reached its limits, and the need for the parallelization of tasks across many CPU cores, in Graphical Processing Units (GPUs), or in other specialized hardware like Field Programmable Gate Arrays (FPGAs) and Application Specific Integrated Circuits (ASICs) has become necessary. (The choice of technology often depends on the timescale and amount of data to handle). For high-energy physics experiments this means moving beyond the natural parallelization of processing individual data ``events'' (e.g. beam crossings, which are independent of each other) to the parallelization of the algorithms themselves acting upon the data of single event. This requires a new paradigm of coding algorithms to take advantage of the available heterogeneous computing hardware, and thus utilizing industry tools or developing domain specific tools to aid in this parallelization. 

Machine learning algorithms lend themselves well to be distributed on such heterogeneous computing platforms using standard libraries, and thus make a natural and powerful target for trigger applications. The applications include the very specialized and local processing at the front-end of the detector electronics (``edge'' computing) where low-level detector hits are converted into clusters or other higher-level data objects at high frequency and low latency, but also the more global and generalized processing needed to discriminate physics signatures from backgrounds. Machine learning also could potentially be used to go beyond the fixed hand-curated trigger menus used to select physics data at colliders to a novel ``self-driving'' paradigm whereby the trigger system autonomously and continuously learns from the data to more efficiently and effectively filters and selects data from a detector system, as discussed in white paper~\cite{TDAQ-innovations}. Such systems may complement dedicated triggers, searching for specific signatures of Beyond-Standard-Model physics, by performing a general set of anomaly detection that may be sensitive to a wider variety of new physics.

%\subsubsection{Fast Machine Learning in early stage trigger}

Development of machine learning algorithms for use in the trigger and data acquisition systems of future high energy physics experiments is particularly challenging~\cite{fastml_summary}. For example, while ML-based algorithms have proven effective at performing effective data reduction, through both advanced data selection and data compression, to be used in high-luminosity environments of future particle colliders these algorithms must be capable of running in on-detector electronics with latencies on the order of nanoseconds. Future neutrino, dark matter, and astrophysics experiments require latencies on the order of microseconds to milliseconds, and often similarly extreme detector environments.

The design and development of low-latency AI algorithms requires optimization across both physics (\textit{e.g.} selection efficiency, background rejection) and technical performance (\textit{e.g.} latency, resource usage). It's necessary to consider a co-design of hardware and software that gives special attention to the processor element, making use of tools and expertise that can bring a variety of ML algorithms built on large datasets into FPGA and ASIC firmware. Open-source frameworks like \texttt{hls4ml}~\cite{hls4ml} and FINN~\cite{FINN} aim to ease the complexity of firmware programming, which have opened up development and integration of sophisticated AI into high-performance hardware. Continued development of ML frameworks that can aid hardware/software co-design, coupled with (and in many cases driving) improvements in the underlying processor technologies, can open the door to paradigm shift in how future experiments will collect, reduce, and process data.

\subsubsection{Innovative Architectures}

%\subsection{Time Multiplexed or Asynchronous Hardware Trigger Systems}
%\label{sec:if04_async}

For experiments where a processing element of the trigger system must have a complete view of the data from all detectors to perform its function, scalability of the trigger system can be achieved by time multiplexing the data to individual processors. This is natural for software-based trigger levels (CPUs, GPUs) in collider experiments, where data are aggregated in an event builder and sent to a target compute node for processing asynchronously. For a hardware-based synchronous trigger level (FPGAs, ASICs), this can be achieved by sending data from all detector elements for a given time slice (or event)  via links to target processors in a round-robin fashion (``time multiplexing''). This will be necessary for the CRES tritium beta decay experiment, for example, where each compute node must process the data from all receivers in a given time slice.

In collider experiments, trigger data processing in the hardware-based
level is still generally synchronous to the accelerator clock, even if
the processing is time multiplexed. At all stages the data are
processed and registered at a multiple of this frequency in the
digital pipeline, and the event number is implicit by the clock (or
accelerator bunch) counter. However, it is enough to time-stamp data
at the very front end of the detectors with the system clock, and
transmit and process the data asynchronously as traditionally done at
the software-based level~\cite{async-L1}. Effectively the event
builder infrastructure moves to the first level of the trigger
system. This would alleviate the challenge of distributing and
synchronizing a stable, low-jitter, high frequency clock  over the
entirety of a very large and distributed electronics system.
It also has the additional benefit of blurring the lines between the
first level trigger, which typically runs in fast FPGAs, with the
software-based higher levels.
Another avenue
of potential interest in this area is to make use of neuromorphic
computing directly on analog signals.  

%\subsection{Streaming DAQ}
%\label{sec:if04_streaming_daq}

Another innovative approach to solving the data reduction problem for trigger and data acquisition systems is to move away from a pipelined and triggered readout, and instead operate in a more ``streaming" design, where data is encoded with its time and origin~\cite{TDAQ-innovations}. In this model, pioneered by the LHCb experiment for its upgrade but being adopted to some degree as well by the other LHC experiments, event data can be reduced at its source, often through simple thresholding and zero suppression, and then aggregated and streamed to downstream computational and storage elements. There, full- or partial-event filtering and further processing and translation of data into higher-level quantities can be performed in order to achieve the reduction in the data throughput and offline computing. Hybrid designs that combine both traditional trigger-based DAQ for some detector subsystems and streaming-readout for others is also possible. Emphasis on such approaches for upgrades and experiments at future facilities has merit, especially due to its ability to simplify DAQ design.

\subsubsection{Developments in novel readout technologies}

The needs of future detectors continue to push readout, triggering, and data acquisition technologies to operate with growing data rates in more extreme environments. Future kton-scale neutrino and dark matter experiments like DUNE and LZ will produce many petabytes of data per year with intrinsic data rates in excess of TB/s, and require readout systems that can reliably operate in cryogenic temperatures over the long lifetimes of the experiments and minimize radiological material volumes to maintain sensitivity to low-energy interactions. In high-energy collider physics at the HL-LHC or potential future colliders like the FCC-hh, data rates in the hundreds of TB/s are possible from tracking and calorimetry systems, and must be able to withstand high radiation rates and not significantly add to the material budget of the detectors. The fundamental challenge of how to move data from readout electronics to online and offline computing resources requires a commitment to research and development in new and improved technologies.

Core to improvements in DAQ are a combination of reducing the data rate close to the detector, and increasing the data bandwidth for a given material and/or power cost, in the extreme environments required. More sophisticated data reduction techniques in detector electronics may be possible with advances in AI, particularly with improvements in translating low-latency machine-learning-developed compression and triggering algorithms to ASICs~\cite{fastml_summary}. In many cases, like in fast tracking algorithms, correlations across different portions of the detector are necessary to develop effective trigger algorithms, and thus fast, localized, and low-material communication is necessary. Wireless communication technologies are an area of large promise here: microwave-based technologies already show reliable data transmission at the 5 Gb/s scale, and promising future work using free space optics may allow for wireless communication at the Tb/s scale \cite{readout-innovations}. Integration of wireless communication into HEP detector design (like, for future tracking detectors in colliders), could allow for new system designs that exploit localized readout, fast analysis, and triggering to intelligently reduce data volumes.

Technologies to allow greater bandwidth off of the detector also show significant promise~\cite{readout-innovations,readout-links}. Silicon-photonics are an appealing alternative to the current VCSEL-based approaches: they can allow integration of fiber-optic connections directly to sensor modules or readout chips (thus reducing the need for electrical cable connections), commercial devices already show high radiation tolerance, and offer a bandwidth twice that of VCSEL devices with a power consumption that is 20\% less. More promising developments exist in Wavelength Division Multiplexing (WDM), where individual serial links can be transmitted on its own wavelength, reducing the need for data aggregation to maintain high data bandwidth per link. WDM could be used in a design to bring data out of the most extreme radiation environments in colliders more efficiently, allowing for further data reduction in downstream DAQ components.

Notably, the work to develop new readout technologies is often less in design, but more in integration and testing with real detector components in real detector environments. It is important to develop and maintain tools and facilities that can allow for realistic full-system testing of readout electronics and DAQ. 

% placeholder possible section
\subsubsection{Timing}

Time measurements will feature prominently in the next generation of
particle physics experiments and upgrades, including integration into
``4D'' tracking systems and ``5D'' calorimeters
(see~\ref{sec:if06_timing}). Timing helps disentangle the effects of
particle pile-up in hadron collisions, discriminates against
beam-induced backgrounds in a muon collider experiment, and can be
used to separate Cerenkov and scintillation light signals in neutrino
and dark matter experiments. Timing also provides particle ID
information useful for a broad range of experiments, including
sensitivity to any slow beyond-standard-model long-lived
particles. Thus it seems evident that timing information will work its
way into the trigger processing chain to improve its selectivity and
precision of measurements. A particular challenge is the need for
synchronization of data at the ${\cal O}(10)$~ps level or better,
including across large distances in the case of radio-frequency
arrays. 

%\section{Developments in computing and hardware for trigger-based applications}

%\subsubsection{Support for installation, commissioning, integration, and operations}

\subsubsection{Fostering and retaining expertise in TDAQ}

Along with the importance in conducting the R\&D to develop and
ultimately construct innovative trigger and data acquisition systems
for future physics facilities, equally important is to build and
retain the domain knowledge and technical expertise within the
high-energy physics community required to support
this~\cite{TDAQ-innovations}. It can be challenging to recruit and
retain highly skilled personnel to address the specialized and
high-tech needs of our community. Essential technical staff can leave
for higher-paying positions in industry, and younger scientists
specializing in instrumentation may/will find career progression and
promotion a challenge in this field. This is compounded by the
timescale for large experiment facilities from construction through to
the end of operations, which can be decades. Thus it is imperative for
the scientific community to provide career opportunities for such
highly skilled people.  

To facilitate fast machine learning development, it is very important to foster
interdisciplinary collaboration between electrical engineering,
computer science and physics, as people in these fields have valuable
expertise in digital design, machine learning techniques and the
physical problems to be addressed.
Also, as much as possible, work should be preserved in an open source
manner, to be used cross-project and cross-experiment and further
built upon in the future.


However, the needs of particle physics experiments are not always relevant to
industrial partners, which implies that the retention of highly-skilled personnel is made even more
important.
The particle physics community has an interest
in edge cases to typical uses in industry, such as electronics that
perform well under constant bombardment from radiation or in cryogenic
fluids. There's also a need for a high degree of reliability, as many
devices are installed in detectors in areas that are inaccessible for
replacement for decades at a time.  It's important for the community
to continue to follow development in industry and to build strong
collaborative networks, but it is as important to develop resources to
pursue R\&D directions that are specific to use cases in the particle
physics domain. 


As we explore new TDAQ architectures and hardware with increasing
complexity whose performance depends on interactions on a systems
level, a dedicated facility that can support TDAQ design and
development while also offering opportunities for integration testing
across low- and high-level triggering, data readout, data aggregation
and reduction, networking, and storage should be established. While
the necessary support hardware for the facility may be localized, the
participating domain experts should encompass a distributed
community. Given many of the common challenges across physics
frontiers, such a Trigger and Data Acquisition Emulation and
Integration Test Facility should cross experiment and project
boundaries, offering support for emulation of detectors and TDAQ
systems, and the development and maintenance of common hardware,
firmware, and software, and  to support TDAQ R\&D for future
detectors. This facility will develop and maintain an accessible
knowledge-base by enabling and supporting connections and
communication between engineers and scientists in many national and
university labs working within different subfields that encounter
similar problems.

Finally, we note that the success of a detector upgrade or new
experiment ultimately depends not just on the delivery of the new
components, but on the successful installation, commissioning, and
integration of them into the experiment as well as their efficient
operation. This applies to trigger-DAQ as much as any other
instrumentation area.
These tasks need to be well thought out
(preferably as part of the initial proposal to evaluate the overall
cost of a new system) and supported. Lack of attention in any of these
areas can lead to substantial and costly delays as well as a failure
to reach the design goals, which jeopardizes the physics output. Thus
the installation, commissioning, and integration tasks as well as the
long-term operations (until the end of the experiment) must be a
priority.  



\subsection{Micro-Pattern Gaseous Detectors}


\subsubsection{Background}

Gaseous Detectors are the primary choice for cost effective instrumentation of large areas and for continuous tracking of charged particles with minimal detector material. Traditional gaseous detectors such as the wire chamber, Resistive Plate Chamber (RPC), and time projection chamber (TPC) with multiwire proportional chamber (MWPC) readout remain critically important for muon detection, track-finding, and triggering in ongoing and planned major particle physics experiment, including all major LHC experiments (ALICE, ATLAS, CMS, LHCb) and DUNE.

Micro Pattern Gaseous Detectors (MPGDs) are gas avalanche devices with order $\mathcal{O}$(100~\textmu m) feature size, enabled by the advent of modern photolithographic techniques. Current MPGD technologies include the Gas Electron Multiplier (GEM), the Micro-Mesh Gaseous Structure (MicroMegas), THick GEMs (THGEMs), also referred to as Large Electron Multipliers (LEMs), the Resistive Plate WELL (RPWELL), the GEM-derived architecture (micro-RWELL), the Micro-Pixel Gas Chamber (\textmu-PIC), and the integrated pixel readout (InGrid).

MPGDs have already significantly improved the segmentation and rate capability of gaseous detectors, extending stable operation to significantly harsher radiation environments, improving spatial and timing performance, and even enabling entirely new detector configurations and use cases.

In recent years, there has therefore been a surge in the use of MPGDs in nuclear and particle physics. MPGDs are already in use for upgrades of the LHC experiments and are in development for future facilities (e.g., EIC, ILC, FCC, and FAIR). More generally, MPGDs are exceptionally broadly applicable in particle/hadron/heavy-ion/nuclear physics, charged particle tracking, photon detectors and calorimetry, neutron detection and beam diagnostics, neutrino physics, and dark matter detection, including operation at cryogenic temperatures. Beyond fundamental research, MPGDs are in use and considered for scientific, social, and industrial purposes; this includes the fields of material sciences, medical imaging, hadron therapy systems, and homeland security. 

Five commissioned white papers on MPGDs were developed during the 2021 Snowmass decadal survey. These summarize ongoing R\&D on MPGDs~\cite{Dehmelt:2022inw}, the future needs for MPGDs in nuclear physics~\cite{Barbosa:2022zql}, and future needs for MPGDs in three broad areas of particle physics: low-energy recoil imaging~\cite{OHare:2022jnx}, TPC readout for tracking at lepton colliders~\cite{Bellerive:2022wrb}, and tracking and muon detection at hadron colliders~\cite{Black:2022sqi}. A white paper with further details on a proposed TPC tracker for Belle~II was also submitted~\cite{Centeno:2022syq}.

%\paragraph{Recent Developments}

\subsubsection{Key Points}
\begin{itemize}
\item {\bf IF05-1}: Micro-pattern gaseous detectors (MGPDs) constitute an enabling technology that is key for large segments of the future U.S. NP and HEP programs, and which also benefits other communities. MPGDs provide a flexible go-to solution whenever particle detection with large area coverage, fine segmentation, and good timing is required.

\item {\bf IF05-2}: The technology is relatively young and should be advanced to performance limits to enable future HEP experiments. Support of generic and blue-sky R\&D is required to achieve this.
\item {\bf IF05-3}: The global HEP community would benefit from U.S. strategy coordination with the ECFA detector R\&D implementation process in Europe.
\item {\bf IF05-4}: In order to maintain and expand U.S. expertise on MPGDs, The U.S. NP and HEP communities would benefit strongly from a joint MPGD development and prototyping facility in the U.S.
\end{itemize}

\subsubsection{MPGDs: Recent advances, current R\&D, and future needs}

 Recent developments in the field of MPGDs, and the role of the RD51 collaboration, are summarized in Ref.~\cite{Dehmelt:2022inw}. MPGDs were developed to cost-effectively cover large areas while offering excellent position and timing resolution, and the ability to operate at high incident particle rates. Significant development time was invested in optimizing manufacturing techniques for MPGDs, in understanding their operation, and in mitigating undesirable effects such as discharges and ion backflow. The early MPGD developments culminated in the formation of the RD51 collaboration hosted by CERN, which has become the critical organization for promotion of MPGDs and which coordinates all aspects of their production, characterization, simulation and use in an expanding array of experimental configurations. The CERN MPGD Workshop is a source of essential expertise in production methods, mitigation and correction of manufacturing issues, and the development of MPGDs for specific experimental environments. 

An impressive array of MPGDs has been developed, from the initial GEM and Micromegas, now used in a wide variety of applications and configurations, through the more recent ThickGEMs, and microR-Wells with resistive layer(s) to mitigate discharge effects. MPGDs are now also used jointly with other detector elements, for example with optical readout and in liquid Argon detectors. In parallel with MPGD detector development, there has been an important creation of a standardized, general electronics system, the Scalable Readout System (SRS). This system has seen widespread use and is of great utility in allowing integration of a variety of frontend electronics into one data acquisition system. For Snowmass 2021, a number of Letters of Interest were received that illustrate ongoing developments and expansion of use of MPGDs. Submissions on high-precision timing, high-rate applications, expansion of the SRS readout system triggering capabilities, and reduction of ion backflow are summarized in Ref.~\cite{Dehmelt:2022inw}. Many other improvements of MPGDs are being actively pursued. Several of these efforts are commented on below. A detailed, comprehensive summary of expected MPGD needs of planned HEP experiments, versus time, can be found in the 2021 European Committee for Future Accelerators (ECFA) detector research and development roadmap~\cite{Detector:2784893}, specifically in Fig.~1.1.

\subsubsection{MPGDs for nuclear physics experiments}
Many current and future nuclear physics (NP) experiments in the United States have or are implementing MPGDs for tracking and particle identification (PID) purposes. We have summarized the role that MPGDs play in NP experiments, and the R\&D needed to meet the requirements of future NP experiments in Ref.~\cite{Barbosa:2022zql}. Examples include advanced MPGDs for Tracking at the Electron-Ion Collider (EIC), to be built at Brookhaven National Laboratory, which requires its tracking system to have low mass ($ X/X_0 ?1\% $), large area $\mathcal{O}$(1~m$^2$), and excellent spatial resolution $\mathcal{O}$(100~\textmu m). MPGDs such as the GEM, Micromegas, and $\mu$RWELL can meet these requirements. The Facility for Rare Isotope Beams (FRIB) at Michigan State University (MSU) will become the world's most advanced facility for the production of rare isotope beams (RIBs). MPGD technologies play an essential role in the science program's success at FRIB. Applications of MPGD technologies include low-pressure tracking and particle-identification (PID) at the focal planes of magnetic spectrometers, Active-Target Time-Projection-Chambers (TPCs), and TPCs for the detection of exotic decay modes with stopped RIBs. Future spectrometers for NP experiments at the Thomas Jefferson National Accelerator Facility (Jefferson Lab) require large area $\mathcal{O}$(m$^2$),  low mass (X/X$_0 \leq$ 1\%), excellent spatial resolution $\mathcal{O}(100\, $\textmu m), excellent timing $\mathcal{O}$(10 ns), high rate $\mathcal{O}$(1~MHz/cm$^2$) tracking detectors technologies for operation in high background rate and high radiation environment. Only MPGD technologies such as GEMs, Micromegas, or $\mu$RWELL detectors can satisfy the challenges of high performances for large acceptance at reasonably low cost. 

{\bf A dedicated MPGD Development Facility} Currently, the majority of MPGD developers and users in the U.S. rely on production facilities and expertise, diagnostic facilities, and standardized readout electronics associated with the RD51 collaboration and CERN. This significantly slows down the R\&D cycle and limits the speed of innovation in the US. It also means all production for US-led experiments has to be outsourced. A U.S.-based MPGD Center of Excellence is needed and would address this issue. We envision a facility similar in nature to the Gaseous Detector Development (GDD) lab at CERN or the SiDet facility at FNAL. Such a facility would benefit both the nuclear physics and particle physics communities in the US. There are also ample opportunities for commercialization and collaboration with industry. We envision such a facility hosted by one of DOE's National Laboratories, such as Jefferson Lab or Brookhaven National Laboratory.

\subsubsection{MPGDs for recoil imaging in directional dark matter and neutrino experiments}
MPGDs can be used to read out the ionization in low-density gas time projection chambers (TPCs) with exquisite sensitivity and spatial resolution. In the most advanced MPGD TPCs, even individual primary electrons---corresponding to an energy deposit on the order of $\sim$30~eV---can be detected with negligible background from noise hits, and 3D ionization density can be imaged with $\sim$(100~\textmu m)$^3$ voxel size. This new experimental technique, enabled by MPGDs, has a large number of interesting applications in fundamental and applied physics. 

One of the most intriguing applications is to scale up TPCs with MPGD readout to construct a competitive, low-background, high-definition ionization imaging experiment, CYGNUS, which would be directionally sensitive to both dark matter and neutrinos. There is an opportunity here for the US to take the lead and initiate a novel experimental program focused on recoil imaging, with broad scientific scope, one that we have only just started to map out.  Because large areas, $\mathcal{O}$(1000~m$^2$), of MPGDs are required, there are clear synergies with this proposal and the needs in nuclear physics, where MPGDs will be used broadly, and where R\&D, production, and test facilities in the US are also desireable. Other notable applications of recoil imaging include the International Axion Observatory (IAXO), directional neutron detection, the measurement of the Migdal effect, X-ray polarimetry, the detection of rare nuclear decays. Several groups are also exploring TPC designs use high density gases such as SeF$_6$ or argon and can provide the sub-mm to 10~micron resolution, for example via `dual readout' TPCs which can detect both the positive ions as well as the electrons generated by a recoil event. TPCs using gaseous argon could be of interest for studies of the neutrino sector, for example $\tau$-tracking for the study of $\nu_\tau \tau$ charged current interactions. Further detail on the emerging field of recoil imaging can be found in Ref.~\cite{OHare:2022jnx}.

\subsubsection{MPGDs at future high energy physics colliders}

Advances in our knowledge of the structure of matter during the past century were enabled by the successive generations of high energy particle accelerators, as well as by continued improvement in detector technologies. In this context, MPGDs have become a preferred solution for enabling both continuous, low-mass charge-particle tracking in TPCs and large-area muon detection systems. Two of the most prominent MPGD technologies, the GEM and MicroMegas, have been successfully operated in many different experiments, such as Compass, LHCb, and TOTEM.
In addition, the low material budget and the flexibility of the base material makes MPGDs suitable for the development of very light, full cylindrical fine tracking inner trackers at lepton colliders such as KLOE-2 at DAFNE (Frascati, IT) and BESIII at BEPCII (Beijing, CN).

The TPC concept is viewed in particle physics as the ultimate drift chamber since it provides 3D precision tracking with low material budget and enables particle identification through dE/dx measurements with cluster counting techniques. At ILC and CEPC, as well as for Belle II upgrades, TPCs with MPGD readout are key to proposed detector designs~\cite{Bellerive:2022wrb,Black:2022sqi,Centeno:2022syq}.

Gaseous detectors are also the primary choice for cost effective instrumentation of very large areas, with high detection efficiency in a high background and hostile radiation environment, needed for muon triggering and tracking at future facilities.
They can provide a precise standalone momentum measurement or be combined with inner detector tracks resulting in even greater precision. Adding precise timing information ,$\mathcal{O}$(ns), allows control of uncorrelated background, mitigates pile-up and allows detection of extremely long lived particles that behave like slow muons propagating through the  detector volume over a time as long as a few bunch crossings. Scaling up of MPGDs to very large single unit detectors of $\mathcal{O}$(m$^2$), has facilitated their use in muon systems in the LHC upgrades. 
Major developments in the MPGD technology have been introduced for the ATLAS and CMS muon system upgrades, towards establishing technology goals, and addressing engineering and integration challenges. Micromegas and GEM have been recently installed  in the ATLAS New Small Wheel, CMS GE1/1 station respectively, for operation from Run 3 onward, as precise tracking systems. Those radiation hard detectors, able to cope with the expected increased particle rates, exhibit good spatial resolution, $\mathcal{O}$(100 \textmu m) and have a time resolution of 5--10~ns. 
%On the algorithm side, 
In the CMS muon system additional stations, GE2/1 and ME0, based on GEMs with high granularity and spatial segmentation, will be installed to ensure efficient matching of muon stubs to offline pixel tracks at large pseudo-rapidities during HL-LHC operation. 
Several solutions ($\mu$-RWELL, Micro Pixel Chamber ($\mu$-PIC), and small-pad resistive Micromegas were also considered for the very forward muon tagger in the ATLAS Phase-II Upgrade Muon TDR proposal. Here, the main challenges are discharge protection and miniaturization of readout elements, which can profit from the ongoing developments on Diamond-Like Carbon (DLC) technology. The $\mu$-RWELL is the baseline option for the Phase-II Upgrade of the innermost regions of the Muon System of the LHCb experiment (beyond LHC LS4).

Muon systems at future lepton colliders, (ILC, CLIC, CepC, FCC-ee, SCTF) or LHeC, do not pose significant challenges in terms of particle fluxes and the radiation environment. Therefore many existing MPGD technologies are suitable for building future large muon detection systems. On the other hand, the expected particle rates for the muon tracking and triggering at future hadron colliders, such as the FCC-hh, make the existing technologies adequate in most regions of the spectrometers, but require a major R\&D  for the very forward endcap region.
In a multi-TeV muon collider, the effect of the background induced by the muon beam decays is extremely important. A new generation Fast Timing MPGD (FTM, Picosec) is considered to mitigate the beam induced background, by rejecting hits uncorrelated in time. \textbf{Required R\&D} should focus on stable operation of large area coverage, including precision timing information to ensure the correct track-event association, and on the ability to cope with large particle fluxes, while guaranteeing detector longevity using environmentally friendly gas mixtures and optimized gas consumption (gas recirculating and recuperation system). 

\subsection{Calorimetry}
\label{sec:calorimetry}

The IF06 Calorimetry group has considered major issues in present and future calorimetry. Input has been taken from a series of talks, group discussions, LOIs, and White Papers. Here we report on two major approaches to calorimeter systems - Particle Flow and Dual Readout, the critical extra dimension of precision timing, and the development of new materials for calorimeters.  What follows is a distillation of the full Report of the Topical Group on Calorimetry~\cite{White:2022abc}, highlighting the key points and recommendations. 

The primary purpose of electromagnetic and hadronic calorimetry is the measurement of the energy of charged and neutral particles and overall event energy. However, they are also important systems for overall event reconstruction, particle identification and triggering. The physics goals and the experimental conditions at future colliders require technical advances in calorimeter technology to fully exploit the physics potential of these facilities. For future $\ee$ colliders, so-called Higgs Factories, the overall precision of event reconstruction is the main focus, while future hadron colliders at energies and luminosities significantly beyond the HL-LHC impose new challenges in terms of the experimental environment.

\subsubsection{Precision timing}
\label{sec:calorimetry-timing}

The potential for precision timing at the 10ps level or better opens new possibilities for precise event reconstruction and the reduction of the negative effects of challenging experimental environments. Precise timing can directly benefit calorimetry in several ways ranging from detailed object reconstruction to the mitigation of confusion from pile-up. It can also lead to improved performance for both particle flow and duel readout-based calorimeters.

Given these possible performance enhancements, the focus is now on the study of timing implementation both at the device level and the calorimeter system level, together with detailed simulations. A range of possible implementations can be envisaged, addressing the needs of calorimetric measurements, confusion reduction, particle identification, and long-lived particle searches. The timing precision required varies across these applications. R\&D is needed to establish whether an average timing precision can satisfy all the requirements at some acceptable level, or, for instance, dedicated high precision timing components are needed in combination with a general systemwide implementation. 

The actual implementation of timing in calorimeter systems can take a number of forms. Timing information can be collected by all active calorimeter cells which, when implemented in a highly granular calorimeter enables a full five-dimensional reconstruction of shower activity in the detector, with corresponding benefits for pattern recognition, spatial shower reconstruction and separation and energy measurement.  However, the very large number of cells might force a compromise with only a fraction of cells instrumented for timing. A less challenging and expensive solution could be the use of timing layers, for instance before and after the electromagnetic calorimeter, and at certain depths in the hadronic calorimeter.

Careful studies are needed to assess the cost/benefits of possible system designs. Adding timing functionality at both the cell and layer levels has implications for material profiles/sampling ratios, power consumption, system complexity and expanded data volume. 
Due to recent developments a number of possible timing technologies have potential applicability to calorimeter systems. However, significant R\&D is needed to address the realities of these choices and this is seen as a major area of future calorimeter development.
Successful implementation can lead to highly performant calorimeter systems well matched to the demands from both future physics studies and experimental environments.

\subsubsection{Active materials}
\label{sec:calorimetry-materials}

The construction of future calorimeters matched to the demands of high radiation tolerance, the need for fast timing, and constrained cost puts strong requirements on the properties of active calorimeter materials. Suitable materials should therefore combine high density, fast decay time, and good radiation hardness with good optical quality and high light yield. To cope with unprecedented high event rate expected by future experiments, an ultrafast total absorption calorimeter with sub-nanosecond decay time is preferred. A range of inorganic scintillators using rare-earth doping in crystals has been developed possessing many of these desired properties.  However, use of these materials in future large-scale calorimeter systems demands attention to material costs to assure affordability and to radiation hardness for long attenuation length of scintillation light after high radiation dose. Scintillating glass is a new type of active material that is being engineered to have similar performance and radiation hardness to lead tungstate. Work continuing to scale up production to the sizes needed for large electromagnetic calorimeter in a cost-effective way is in progress. 

Organic-based scintillator calorimeters, including plastics scintillator, liquid scintillator, and water-based liquid scintillator, have fast pulse response with comparable light-yield to inorganic crystals. The plastic scintillators, polyvinyltoluene or polystyrene base, have seen very wide use, having the advantages of ease of use and relatively low cost.  A new thermoplastics acrylic scintillator aiming to load scintillator materials and high-Z elements directly into acrylic monomers is under development. The combination of plastic scintillators with SiPM readout has significantly expanded the flexibility of calorimeter design.  An alternative method to fabricate plastic detectors with tight controls on shape and dimension using a computer-aided 3D-printing design is highly desired. Finally, liquid scintillators have very low unit cost with improved properties in terms of stability and material compatibility that have been largely advanced through neutrino and other rare-event physics over the past decade and been widely used where very large volumes (10s of kilotons) are required.  An interesting development is the potential of metal doped (water-based) liquid scintillators for use as active materials in sampling calorimeters.

\subsubsection{Particle flow}
\label{sec:calorimetry-PF}

Particle flow calorimetry makes use of the associations of charged tracks and calorimeter energy deposits to achieve precise reconstruction of hadronic jets and measurement of their energy. Such associations can aslo be effectively used to reduce the effects of pileup. Implementation of a PFA-based calorimeter requires a small cell size and high granularity leading to very high channel counts. Challenges remain in realizing calorimeter systems with up to 100 million cells. Developent is onging for such systems in the areas of power (heat) management, integration of on-board ASICs, and components of signal extraction. A variety of approaches to PFA calorimeters are under developent ranging from scintillator-SiPM systems to a range of gas-based systems using GEMs, Micromegas and RPCs. Also being explored are the potential benefits of precise timing (see above) and moving some elements of a PFA into the front-end electronics.

The HEP community has demonstrated its strong interest in pursuing this technology in multiple applications in various stages of development.  These include the HL-LHC (CMS HGCAL), $\ee$ collider alternatives (SiD and ILD for the ILC, the CLIC detector concept, CLD for the FCC-ee, and the baseline CEPC detector concept), FCC-hh, and a possible muon collider.  Among these, the CMS HGCAL upgrade for the HL-LHC is at the most advanced stage of development, with delivery of the production silicon sensors slated to begin in January 2023.  The HGCAL will be a crucial demonstration of the particle flow concept.  Lessons learned from the assembly, operation, and PF reconstruction of the HGCAL will influence simulation techniques, design, and costing for future PF calorimeters, and will reveal the areas in which R\&D is most needed.

PF calorimetry development has synergies with developments in other areas of HEP instrumentation.  Silicon detectors, SiPMs, fast scintillators, and gas ionization detectors are all good candidate active media, depending on the use case.  Smart, low-power, radiation-tolerant front end electronics are needed to realize compact designs.  PF reconstruction provides a benchmark for optimizing novel computational methods, like the use of machine learning in triggering or particle reconstruction.  The computational problem of particle flow reconstruction, in which charged and neutral hadrons, electrons, muons, hadronic tau decays, photons, and jets must be identified from associations between tracks and highly granular calorimeter deposits, may be particularly well suited to machine learning methods as opposed to a traditional deterministic algorithm.  In turn, PF reconstruction requires performance advances that can speed up detector simulation or improve jet energy resolution.  Breakthroughs in any of these related technologies can drive significant progress in PF calorimetry, be it cost reduction, simplification of engineering, increased radiation hardness, or improved physics performance.

To realize the full potential of PF calorimetry, and to ensure that it is ``shovel-ready'' when the next large experiment is approved, R\&D is needed to solve outstanding problems.  Extensive beam testing, especially of large-scale technological prototypes, is needed to study integration issues and how they affect electromagnetic and hadronic energy resolution.  As stated above, more research is needed in front end design, especially for high occupancy and high radiation applications like a future hadron or muon collider.  Finally, the challenge of rethinking traditional assembly and QA/QC procedures to find solutions that scale to tens to hundreds of millions of channels cannot be overlooked.  There is a growing need to incorporate lessons from product and process engineering into instrumentation labs, either through personnel decisions or by adapting the training of traditional physics graduate students and postdocs.  Similarly, academic-industrial partnerships need to be formed with this scale in mind.

\subsubsection{Dual readout}
\label{sec:calorimetry-DRO}

The dual readout approach to the precise measurement of jet energies makes use of the scintillation light and 
Cerenkov light from showers. The relative amounts of scintillation and Cerenkov light is used to correct the shower energy. The original approach to implementing dual readout calorimetry used a matrix of scintillating fibers and clear optical fibers (for the Cerenkov component) in a block of absorber material. However, with the reduced need for spatial associations (as in particle flow), dual readout can make beneficial use of an electromagnetic front section using homogeneous scintillating crystals which have excellent electromagnetic energy resolution. Development of dual readout systems has followed both of these approaches. In the second case, the separation of the scintillation and Cerenkov signals can be achieved by the use of optical filters and SiPM readout and/or exploitation of the different time structure of the two signals. Development and testing of large-scale systems is needed to demonstrate the feasibility of both the all-fiber and homogeneous electromagnetic section plus fibers approaches to dual readout.

Significant R\&D is still needed to fully realize the potential of DRO.  Large-scale prototypes need to be constructed to understand which parts of the engineering are cost drivers, which need further R\&D, and how a realistic system will perform.  Such efforts have already begun in the context of $\ee$ circular collider studies.  The Innovative Detector for an Electron-positron Accelerator (IDEA) fiber calorimeter considers a stacked capillary arrangement as well as a 3D-printed copper alveolar tower into which fibers are inserted.  In the case of homogeneous scintillating crystals, a key open question is how to ensure that readout of the red end of the $\check{\mathrm{C}}$erenkov spectrum, far from the scintillation peak, will yield a large enough signal with which to perform the DRO correction.  Due to the large size of collider detectors, another important question is how to drive down the cost of high-performing crystal scintillators.  In the long term, research into new optical materials, such as photonic crystal fibers for increased $\check{\mathrm{C}}$erenkov light collection, quantum dot and semiconductor nanoparticle wavelength shifters, and fibers that maintain polarization information, can improve the performance and/or reduce the cost of DRO fiber calorimeters.

The wide availability of high performance SiPMs serves to simplify DRO mechanical design and allows for channel granularity not initially envisioned.  There is no reason that the advantages of PF and DRO cannot be combined in certain applications to yield even more flexibility.  Readout of each fiber by a SiPM opens the door to jet imaging and position reconstruction using algorithmic or deep learning techniques.  This can enable gluon/jet discrimination, studies of jet substructure, or identification of tau leptons or boosted objects.  Indeed, the extra front end information that DRO relies on requires advances in electronics for efficient processing and reduction.  Areas of R\&D in this direction include system-on-chip waveform digitizers with real-time analysis, field programmable analog arrays on the front end, and digital SiPMs.  With flexibly designed readouts, it may also be possible to use the time structure of the $\check{\mathrm{C}}$erenkov and scintillation signals to estimate the shower EM fraction online and improve triggering.

\subsubsection{Summary and recommendations}
\label{sec:calorimetry-summary}

The field of calorimeter research and development remains very active. The precision energy measurement requirements of future physics programs is stimulating innovation in the particle flow and dual readout systems.  The increasing availability of precise timing is adding an important new dimension to system implementation, while the development of a range of fast, radiation-hard active materials is leading to increased flexibility and exciting possibilities for calorimeter system designs.

\begin{itemize}
\item[\bf IF06-1] Future calorimetry at fixed target and colliding beam experiments should be \textbf{fundamentally multidimensional}, providing shower position, time, energy, and a detailed look at shower constituents through the exploitation of an application-specific \textbf{combination of particle flow techniques, materials with intrinsically good time or energy resolution, and/or dual readout techniques.} R\&D support is needed to achieve these goals.
\item[\bf IF06-2] Sustained R\&D is needed to move multidimensional calorimetry \textbf{from prototype to realistic detector.}  Scaling to hundreds of thousands or tens of millions of channels while maintaining the required quality is a huge challenge.
\item[\bf IF06-3] \textbf{Electronics must be developed to allow new features} such as fast timing \textbf{without significantly adding to the power budget or cooling load.} It will be necessary to have \textbf{HEP personnel trained in the new technologies} and close tracking of new electronics options emerging in industry.
\item[\bf IF06-4] \textbf{Effective partnerships} with chemists, materials scientists, industries large and small, and radiation facilities must be continued and strengthened to \textbf{explore the landscape of materials} that enable precision calorimetry and to lower the cost.
\end{itemize}

% Future calorimetry at fixed target and colliding beam experiments will be fundamentally multidimensional, providing shower position, time, energy, and a detailed look at shower constituents through the exploitation of an application-specific combination of particle flow techniques, materials with intrinsically good time or energy resolution, and/or dual readout techniques. Sustained R\&D support is needed to achieve this and to move multidimensional calorimetry from prototype to realistic detector.  Scaling to hundreds of thousands or tens of millions of channels while maintaining the required quality is a huge challenge.  Electronics must be developed to allow new features such as fast timing without significantly adding to the power budget or cooling load. It will be necessary to have HEP personnel trained in the new technologies and close tracking of new electronics options emerging in industry.  Finally, effective partnerships with chemists, materials scientists, industries large and small, and radiation facilities must be continued and strengthened to explore the landscape of materials that enable precision calorimetry and to lower the cost.

% Text prior to 2-Sep-22 commented out by RPY and replaced with latest version above
% The IF06 Calorimetry group has considered major issues in present and future calorimetry. Input has been taken from a series of talks, group discussions, LOIs, and White Papers. Here we report on two major approaches to calorimeter systems - Particle Flow and Dual Readout, the critical extra dimension of precision timing, and the development of new materials for calorimeters. 

% The potential for precision timing at the 10ps level or better opens new possibilities for precise event reconstruction and the reduction of the negative effects of challenging experimental environments. Precise timing can directly benefit calorimetry in several ways ranging from detailed object reconstruction to the mitigation of confusion from pile-up. It can also lead to improved performance for both particle flow and duel readout-based calorimeters.
% Given these possible performance enhancements, the focus is now on the study of timing implementation both at the device level and the calorimeter system level. Successful implementation can lead to highly performant calorimeter systems well matched to the demands from both future physics studies and experimental environments.

% The construction of future calorimeters matched to the demands of high radiation tolerance, the need for fast timing, and constrained cost puts strong requirements on the properties of active calorimeter materials. Suitable materials should therefore combine high density, fast decay time, and good radiation hardness with good optical quality and high light yield. A range of inorganic scintillators has been developed possessing many of these desired properties. However, use of these materials in future large-scale calorimeter systems demands attention to material costs to assure affordability. Organic based plastic scintillators have seen very wide use, having the advantages of ease of use and relatively low cost. The combination of plastic scintillators with SiPM readout has significantly expanded the flexibility of calorimeter design. Finally, liquid scintillators, with low unit cost, have been widely used where very large volumes are required. An interesting development is the potential of metal doped (water-based) liquid scintillators for use as active materials in sampling calorimeters. 

% Particle flow calorimetry makes use of the associations of charged tracks and calorimeter energy deposits to achieve precise reconstruction of hadronic jets and measurement of their energy. Such associations can aslo be effectively used to reduce the effects of pileup. Implementation of a PFA-based calorimeter requires a small cell size and high granularity leading to very high channel counts. Challenges remain in realizing calorimeter systems with up to 100 million cells. Developent is onging for such systems in the areas of power (heat) management, integration of on-board ASICs, and components of signal extraction. A variety of approaches to PFA calorimeters are under developent ranging from scintillator-SiPM systems to a range of gas-based systems using GEMs, Micromegas and RPCs. Also being explored are the potential benefits of precise timing (see above) and moving some elements of a PFA into the front-end electronics.

% The dual readout approach to the precise measurement of jet energies makes use of the scintillation light and Cerenkov light from showers. The relative amounts of scintillation and Cerenkov light is used to correct the shower energy. The original approach to implementing dual readout calorimetry used a matrix of scintillating fibers and clear optical fibers (for the Cerenkov component) in a block of absorber material. However, with the reduced need for spatial associations (as in particle flow), dual readout can make beneficial use of an electromagnetic front section using homogeneous scintillating crystals which have excellent electromagnetic energy resolution. Development of dual readout systems has followed both of these approaches. In the second case, the separation of the scintillation and Cerenkov signals can be achieved by the use of optical filters and SiPM readout and/or exploitation of the different time structure of the two signals. Development and testing of large-scale systems is needed to demonstrate the feasibility of both the all-fiber and homogeneous electromagnetic section plus fibers approaches to dual readout.

% The field of calorimeter research and development remains very active. The precision energy measurement requirements of future physics programs is stimulating innovation in the particle flow and dual readout systems.
% The increasing availability of precise timing is adding an important new dimension to system implementation, while the development of a range of fast, radiation-hard active materials is leading to increased flexibility and exciting possibilities for calorimeter system designs.

\subsection{Readout Electronics and ASICs}
In pursuit of its physics goals, the high energy physics community
develops increasingly complex detectors, with each subsequent
generation pushing to ever finer granularity. For example, the
emergence and growing dominance 
of particle-flow reconstruction methods has stressed
the increasing importance of very fine detector granularity, not
only for tracking detectors but also for calorimetry, and has also
initiated the push to "4D" detectors that combine precision measurements
of both spatial and time coordinates to their measurements of
energy and momentum. While these development have led to enormous
growth in detector channel counts, the analog performance requirements 
for energy and momentum measurements, as well as spatial and timing precision, are being maintained or (more typically) even tightened.

These
challenging detector requirements push the corresponding development of
readout electronics. A variety of factors, including the growing
specialization of the functionality required, and the explosive
growth in channel counts and typically modest (if any) increases in the
material budget and the power and cooling budgets,
lead to the increasing reliance on custom-developed Application
Specific Integrated Circuits (ASICs). This trend is further 
exacerbated by challenges in the various experimental environments,
including radiation hardness requirements, cryogenic 
and deep-cryogenic operations, and 
space-based detector systems.
The development of custom ASICs in advanced technology nodes allows HEP detector
subsystems to achieve higher channel density, enhanced
performance, lower power consumption, lower mass, much greater radiation
tolerance, and improved cryogenic temperature performance than is possible
with commercial integrated circuits (ICs) or discrete components. 
The higher level of integration also leads to fewer components and
fewer connections, leading to higher reliability, as required by
experiments that can run for decades and that provide access to
the on-detector electronics at most annually, and sometimes never.

This writeup summarizes the work of ``IF07'', namely
Topical Working Group 7 of the
Instrumentation Frontier group of the Snowmass 2021 process. Group IF07
dealt with issues pertaining to ASICs and Readout Electronics. The
community efforts as part of IF07 were organized across 7 white papers
submitted to the Snowmass process. The first~\cite{whitepaper1}
discusses issues related to the need to maintain the talented
workforce required to successfully develop future HEP electronics
systems, and to provide the appropriate training and recruitment.
The remaining papers focused on electronics for particular detector
subsystems or technologies, including calorimetry~\cite{whitepaper2},
%silicon- and photo-detectors~\cite{whitepaper3},
detectors for fast timing~\cite{whitepaper4},
optical links~\cite{whitepaper5},
smart sensors using AI~\cite{whitepaper6},
%cryogenic readout~\cite{whitepaper7},
and RF readout systems~\cite{whitepaper8}. In the following
section, a brief overview is provided of each 
of the white papers in turn.  
A white paper on silicon and photo-detectors was originally considered. This content is now captured by other frontiers with contributions form ASICs and readout electronics.

The interested reader is referred to the white papers themselves, and to the references each contains, for a more detailed discussion of each of the various topics.

%***write a few sentences of high-level listing of important issues?? See added below

There are some overarching goals for advancing the field of readout and ASICs. Among those three activities with broad impact are:
1) Provide baseline support and specialized training opportunities for the instrumentation work force to keep the US electronics instrumentation \& ASIC  workforce;
2) improve mechanisms for access to advanced technology;
3) continue to develop methodologies to adapt the technology for operation in extreme environments;
4) expand framework and platform for easy access to design tools.

\subsection{Noble Elements}
Particle detectors making use of noble elements in gaseous, liquid, or solid phases are prevalent in neutrino and dark matter experiments and are also used to a lesser extent in collider-based particle physics experiments. These experiments take advantage of both the very large, ultra-pure target volumes achievable and the multiple observable signal pathways possible in noble-element based particle detectors. As these experiments seek to increase their sensitivity, novel and improved technologies will be needed to enhance the precision of their measurements and to broaden the reach of their physics programs. The priority research directions (PRDs) and thrusts identified in the 2019 Report of the Office of Science Workshop on Basic Research Needs for HEP Detector Research and Development (BRN report)~\cite{osti_1659761} are still relevant in the context of this Snowmass 2021 topical group. The areas of R\&D in noble element instrumentation that have been identified by the HEP community in the Snowmass whitepapers and Community Summer Study align well with the BRN report PRDs, and are highlighted by five key messages (with IF-wide themes in bold):
\begin{itemize}
    \item[\bf IF08-1] Enhance and combine existing modalities (scintillation and electron drift) to {\bf increase signal-to-noise and reconstruction fidelity}.
    \item[\bf IF08-2] {\bf Develop new modalities for signal detection} in noble elements, including methods based on ion drift, metastable fluids, solid-phase detectors and dissolved targets. Collaborative and blue-sky R\&D should also be supported to enable advances in this area.
    \item[\bf IF08-3] Improve the understanding of {\bf detector microphysics} and calibrate {\bf detector response in new signal regimes}.
%    \item {Advance material purification and assay methods to increase sensitivity}
    \item[\bf IF08-4] {\bf Address challenges in scaling technologies}, including material purification, background mitigation, large-area readout, and magnetization.
    \item[\bf IF08-5] {\bf Train the next generation of researchers}, using fast-turnaround instrumentation projects to provide the design-through-result training no longer possible in very-large-scale experiments.
\end{itemize}

The IF08 topical group report~\cite{Dahl:2022bst} identifies and documents recent developments and future needs for noble element detector technologies. In addition, we highlight the opportunity that this area of research provides for continued training of the next generation of scientists.

%\begin{figure}[htb]
%\begin{center}
%\includegraphics[width=\textwidth]{SnowmassBook_IF/Instrumentation/IF08/figures/IF08SummaryFig.pdf}
%\caption{Summary of the multiple physics goals (shaded regions) targeted by noble element detectors and the %variety of detector technologies (boxes) used to meet those goals, with relevant energy ranges and detector %sizes indicated.  The efforts described in the IF08 topical group report~\cite{Dahl:2022bst} aim to extend the %reach (arrows) and improve the performance (angle boxes) of these detectors.}
%\end{center}
%\end{figure}

\subsection{Radio Detection}


\subsubsection{IF 10: Executive Summary}
Detection techniques at radio wavelengths
play an important role in the future of 
astrophysics experiments.
The radio detection of cosmic rays, neutrinos, and photons has emerged as the technology of choice at the highest energies.   Cosmological surveys require the detection of radiation at mm wavelengths at thresholds down to the fundamental noise
limit.

High energy astroparticle and neutrino detectors use large volumes of a naturally occurring suitable dielectric: the Earth's atmosphere and large volumes of cold ice as available in polar regions.
The detection technology for radio detection
of cosmic particles has matured in the past decade and is ready to move beyond prototyping or midscale applications. 
Instrumentation for radio detection has reached a maturity for science scale detectors. 
Radio detection provides competitive results in
terms of the measurement of energy and direction and in particle identification when to compared to currently applied technologies for high-energy
neutrinos when deployed in ice and for
ultra-high-energy cosmic rays, neutrinos, and
photons when deployed in the atmosphere.  It 
has significant advantages in terms of cost per
detection station and ease of deployment.
%The optical technique has already been successfully implemented in large scale detectors in ice (IceCube), and efforts are projects underway to apply them in large scale in water (km3NeT, Baikal-GVD).
%IceCube is preparing an upgrade  that will increase the sensitivity by a factor of 5 to 10 driven by optical detectors and by 2 orders of magnitude driven by the radio detection technique (E $>$ 100 PeV)
%The option to detect earth-skimming neutrinos with optical Cherenkov telescopes is being explored. 



\begin{itemize}
%     \item  IF10-1  IceCube-Gen2~\cite{IF-022-Karle}
%  has developed a conceptual design that will be released as a Technical Design Report later this year. Further investment in R\&D can potentially reduce cost and optimize design. 
%     \item IF10-2  Opportunities exist in optimizing for power and simplifications: eg ASIC based digitizer/readout (PMT) or RFSoC (Radio Frequency System on Chip).  Investigate if synergies with experimental needs in other areas exist.
%     \item IF10-3  Remote power and communications approaches of very large extended  arrays  can still benefit from dedicated R\&D. Explore synergies with other experiments, like DUNE, SKA, CTA, which also need large distance communication and synchronization.
\item IF10-1  While conceptual designs exist for next-generation arrays, investment in R\&D can reduce cost and optimize designs.
\item IF10-2  Opportunities exist in optimizing for power and simplifying: e.g. by using ASIC-based digitizer/readout  or RFSoCs (Radio Frequency System on Chip).  Investigations are needed to identify synergies with experimental needs in other areas.
\item IF10-3  Remote power and communications approaches of very large extended arrays can still benefit from dedicated R\&D. Explore synergies with experiments in other areas, like DUNE, SKA, CTA, which also need large distance communication and synchronization.
\item IF10-4  Enable future mm-wave cosmic probes through R\&D and pathfinder experiments of new mm-wave detectors with higher channel density relative to current CMB detectors.
\end{itemize}


\subsubsection{Radio detection of cosmic particles}

Astrophysical neutrinos, cosmic rays, and gamma rays are excellent probes of astroparticle physics and high-energy physics
~\cite{NF-04-Ackerman}. High-energy and ultra- high-energy cosmic particles probe fundamental physics from the TeV scale to the EeV scale and beyond.

Radio detection offers opportunities to
instrument large areas on the surface of the earth.
This is important because at
energies above an EeV, the cross section for
neutrinos interacting with matter have increased
so much that the detector area becomes a more
important parameter for the acceptance then
the fiducial volume.  At these energies, the 
preferred conversion targets for the neutrinos
are mountains, the earth's crust, ice, or even the
atmosphere.  
For ultra-high energy cosmic rays and photons,
radio detection utilizes the air shower formed in the atmosphere.


While the optical Cherenkov technique has been enormously successful in
measuring neutrinos from $\mathcal{O}$({MeV}) to $\mathcal{O}$(10\,{PeV}), 
%and there is no alternative to it in this energy range. 
at higher energies, techniques at radio frequencies are the most promising for neutrino detection. 
In the energy range from 10 TeV to 30 PeV a factor of 5 in increase 
of sensitivity is needed in order to move from the discovery of cosmic 
neutrinos and the first correlation with sources to 
identify the sources of the cosmic neutrino flux and explore fundamental physics 
with high energy neutrinos. 

Like in the optical, for radio techniques the two media being pursued broadly are the atmosphere and solid natural ice, the latter with emphasis on neutrinos. Both can be used to pursue science with cosmic rays, energetic neutrinos, or both.  
Above about 100\,PeV, volumes of order 1000\,km$^{3}$, which can only be naturally occurring, are
necessary to detect the rare astrophysical neutrino flux in this regime.  Volumes of this scale are too large to instrument with the tens-of-km spacing necessary for optical sensors. 
This spacing of optical is set by the distance over which optical light is absorbed or scattered in the glacial ice that is used as the detection medium.  
However, clear ice is transparent
to radio-frequency signals over distances
of order 1\,km, which sets the 
typical spacing for  detectors
using radio techniques.  

 


There are many
different approaches to the detection
of cosmic particles at radio frequencies~\cite{NF-04-Wissel}.  These approaches, the instrumentation that is unique and common to each, and
future developments are described in this section.




\subsubsection{Askaryan}

In matter, particle cascades induced by cosmic particles produce Askaryan emission. The emission comes about
from the time evolution of a charge
asymmetry that develops in these particle 
cascades by ionization electrons moving with the
cascade's front and positive ions staying behind.  
It is coherent
for frequencies up to about 1\,GHz when viewed
at the Cherenkov angle
and is linearly polarized perpendicular to
the cascade direction and inward to its axis.
Askaryan emission was measured in test beam
experiments in the 2000s.  It has also been observed
to be emitted from cosmic ray air showers.
 Now, many
experiments are
searching for this signature from 
ultra-high energy neutrino interactions 
either from within the ice or by viewing ice from altitude.



\subsubsubsection{In-ice}

One approach to detecting neutrinos via
the Askaryan signature is by embedding
antennas into the ice itself, and the
first experiment to take this approach
was RICE.  Since then, ARIANNA, ARA, and
RNO-G~\cite{NF-04-RNOG-Wissel} search for ultra-high energy 
neutrinos with antennas deployed
in the ice, either at shallow depths (within $\sim$10\,m of the surface) or somewhat deeper (up to 200\,m).  An integrated facility for 
a wide band neutrino detector is IceCube-Gen2 that will employ both optical and radio detectors.  Deep detectors are
employing interferometry-based trigger designs.



% These experiments have sensitivity to all three
% flavors [136, 137], and may have power to discriminate flavor based on different event topologies [137, 138].
% ARA [139] and ARIANNA [140] (and the planned ARIANNA-200 [141]) consist of radio antennas buried in the
% Antarctic ice. RNO-G is a planned radio detector in Greenland, currently under development [142]. IceCube-
% Gen2 will include an expansive, sparse radio array, building on the experience gained in these experiments [132].

\subsubsubsection{Balloon}

Another approach to detecting the
Askaryan signature from ultra-high energy 
neutrinos is to deploy antennas on 
a balloon-borne
payload at stratospheric altitudes where
the payload can view 
approximately 1.5\,million km$^2$ of ice.
At these altitudes, the threshold for a detection
is higher, but above threshold, balloons greatly exceed
ground-based approached in viewable area.
The ANITA project flew four times
under NASA's long-duration balloon
program, and the next-generation PUEO~\cite{NF-04-Vieregg}
is set to launch in the 2024-2025 Austral 
summer season with a trigger that will use an interferometric
approach.

\subsection{Geomagnetic emission}


A cosmic ray incident on the atmosphere will
produce a particle cascade, and charges in
the cascade produce a transverse current due to the earth's magnetic field, which produces 
what is known as geomagnetic emission at radio
frequencies.  The geomagnetic emission is coherent
up to frequencies of about 1\,GHz
and is linearly polarized perpendicular to both the
earth's magnetic field and cascade direction.
The Askaryan emission mentioned above also
contributes to the radio frequency signal from
air showers on average at the 20-30\,\% level in energy
density.  The interplay between geomagnetic
and Askaryan emission gives rise to a non-azimuthally symmetric signal pattern due to
the interplay of the different radiation patterns.
Both are collimated in a Cherenkov cone with
an opening angle of typically a degree.

A next generation ultra-high energy cosmic
particle observatory is required to exploit 
proton astronomy and to discover ultra-high
energy neutrinos and photons.  Such a next-generation cosmic particle observatory
needs to cover a large area, up to 200,000\,km$^2$.
Radio detection is the current favorite to make
deployment at this scale possible and GRAND
proposed to cover an area of this size.





\subsubsection{Radio detection of cosmic rays}

In addition to the traditional strategies
for detecting high energy cosmic rays incident on
the atmosphere, which include detection
of secondary particles, optical Cherenkov
emission, and fluorescence emission,
geomagnetic emission is a strategy that
complements the others and
has seen major advancements in the past two decades
~\cite{CF-07-Schroeder}.  Radio detection of cosmic rays
has a round-the-clock duty cycle and leaves
a broad ($\sim 100$\,m) footprint on the ground.




\subsubsection{Detection of neutrino-induced, earth-skimming air showers}

The combined geomagnetic and Askaryan signatures can also be used to 
detect air showers that can originate from
energetic tau neutrinos that are earth skimming~\cite{CF-07-Abraham}.  These can produce a tau
lepton through a charged current interaction
in matter, and the tau can subsequently decay to produce an electromagnetic or hadronic shower.  


The detection of pulses consistent with air showers going in the upward
direction  has the advantage of being flavor sensitive, and has become an objective of many 
detectors.
BEACON~\cite{CR-07-Wissel}, in prototype phase, TAROGE, and TAROGE-M are compact antenna arrays in elevated locations that aim to detect UHE $\nu_{\tau}$ emerging upwards via the radio emission of the air showers that they trigger. ANITA  and PUEO  are also sensitive to upgoing $\nu_{\tau}$ , from a higher elevation. GRAND~\cite{NF-04-Bustamante} is a planned experiment that will cover large areas with a sparse antenna array to detect the radio emission from air showers triggered by UHE 
$\nu_{\tau}$, cosmic rays, and gamma rays.
This is also a neutrino signature for PUEO, the
follow-up of ANITA, and many other dedicated projects instrumenting large areas with
antennas such as GRAND or putting them in mountains such as BEACON
and TAROGE.




\subsubsection{RADAR}

An alternate strategy for detection
of neutrinos at radio frequencies uses RADAR~\cite{IF10-Prohira}.
When a high-energy neutrino interacts in the ice, it produces a relativistic cascade of charged particles that traverse the medium. As they progress, they ionize the medium, leaving behind a cloud of stationary charge. This cloud of charge, which persists for a few to tens of nanoseconds, is dense enough to reflect radio waves. Therefore, to detect a neutrino, a transmitter can illuminate a volume of dense material like ice, and if a neutrino interacts within this volume, the transmitted radio will be reflected from the ionization cloud to a distant receiver, which monitors the same illuminated volume.

With this technique, a custom signal is transmitted in the ice and received 
after reflections from neutrino-induced
cascades.  With this technique, the
experimenter can determine the properties
of the signal (including the amplitude,
up to what is permitted to be transmitted).
Also, the radar method has excellent geometric acceptance relative to passive 
(Askaryan) methods, which require the detector to lie within a small angular window 
at the Cherenkov angle.  Recent test beam measurements have demonstrated the feasibility of the method in the laboratory, with in-situ tests forthcoming. RET-CR will serve as a pathfinder experiment, and RET-N could make radio detections of UHE neutrinos within the decade with the potential to complement or improve upon existing technologies in this
energy regime.

% For a station consisting of a single, central 40 kW transmitter and 27 receiving antennas out radially from this transmitter, RET-N is projected to probe some flux models. For 10 such stations, the sensitivity at 10 PeV is projected to be comparable to IceCube, with the potential to complement or improve upon existing technologies at higher energies, allowing RET-N to continue detection of the neutrino spectrum beyond the optical regime.




\subsection{KIDs}

Cosmological surveys require the detection of radiation at mm wavelengths at thresholds down to the fundamental noise
limit.  The detection of mm-wave radiation is
important for: studying cosmic acceleration (Dark Energy) and testing for deviations from general relativity expectations through measurements of the kinetic Sunyaev-Zeldovich effect, precision cosmology (sub-arcminute scales) and probing new physics through ultra-deep measurements of small-scale CMB anisotropy, and mm-wave spectroscopy to map out the distribution of cosmological structure at the largest scales and highest redshifts.

Imaging and polarimetry surveys at sub-arcminute scales will require O($10^6$) detectors over a O(10 deg$^2$) fields-of-view (FoV) covering 9 spectral bands from 30\,GHz to 420\,GHz. Spectroscopic surveys (over a smaller FoV initially, O(1\,deg$^2$), but potentially also reaching O(10\,deg$^2$)) will require a further factor of 10–100 increase in detector count.
The 2019 report of the DOE Basic Research Needs Study on High Energy Physics Detector Research and Development 
identified the need to carry out detector R\&D to 
achieve this goal.
The driver for new technology is not the detector count
but the increased detector {\it density}.   Whereas in
current experiments, the detector packing density is
limited by the physical size of elements in
existing demonstrated multiplexing schemes, KIDs
eliminate the need for additional cold multiplexing
components, allowing for arrays at the densities needed
for the science aims of proposed cosmological surveys.

The kinetic inductance detector (KID) is a technology that has gained significant traction in a wide range of applications across experimental astronomy over the last decade. A KID is a pair-breaking detector based on a superconducting thin-film microwave resonator, where the relative population of paired (Cooper pairs) and un-paired (quasiparticles) charge carriers govern the total complex conductivity of the superconductor. Photons with energy greater than the Cooper pair binding energy (2$\Delta$) are able to create quasiparticle excitations and modify the conductivity. By lithographically patterning the film into a microwave resonator, this modification is sensed by monitoring the resonant frequency and quality factor of the resonator.
Since each detector is formed from a microwave resonator with a unique resonant frequency,  a large number of detectors can be readout without the need for additional cryogenic multiplexing components.  In addition, the designs to be fabricated are 
relatively simple.

There are a number of KID-based architectures being developed  for a variety of scientific applications.  Direct Absorbing KIDs are
the simplest variant, where the resonator geometry is optimized to act as an impedance-matched absorber to efficiently collect the incoming signal.  To date, the only facility-grade KID-based instruments are based on this detector architecture, with the NIKA-2 experiment on the IRAM 30-meter telescope having demonstrated that the KID-based instruments are highly competitive with other approaches.  Microstrip-coupled KIDs take
advantage of recent advancements that
allow for
the ability to lithographically define 
circuits capable of on-chip signal processing with extremely low loss.  The capability
to robustly couple radiation from superconducting thin-film microstrip 
transmission lines into a KID with high optical efficiency is being developed.
Thermal Kinetic Inductance Detectors take
a similar approach as has been developed
for bolometric transition edge sensor arrays.
Instead of directly absorbed radiation breaking pairs, a thermally-mediated KID (TKID) uses the intrinsic temperature response of the superconducting film to monitor the temperature, and therefore absorbed power.
It combines the multiplexing advantage of
KIDs with the proven performance of bolometric designs in TES detectors, at the expense of fabrication complexity.

On-chip spectroscopy is a
natural extension of multi-band imaging using on-chip filters  to a filter-bank architecture to realise medium-resolution spectroscopic capability.  Several approaches to on-chip spectroscopy exist at a range of technological readiness.



% \section{Integrated Optical Cherenkov and Radio detection.}
% We briefly address here the optical Cherenkov method and the integrated approach 
% of IceCube-Gen2. 
% IceCube has been very successful in observing a cosmic flux of neutrinos of all flavors in the energy range from 10\,GeV to 10 PeV.  
% Currently the IceCube Collaboration is building instrumentation to deploy an upgrade of 7 densely instrumented strings optimized for low energies and precision calibration of IceCube. The completion of this upgrade planned for January 2026. 
% This upgrade also serves as a Phase 1 exercise in designing new instrumentation for IceCube-Gen2 and prepare for a preliminary design.  IceCube-Gen2 will consist of 120 additional strings, which are longer and more widely spaced to instrument a total volume of a factor of 8 times that of IceCube.  At high energies, IceCube-Gen2 will be complemented by a radio detector array covering an area of about 500\,km$^{2}$ which will surpass the optical array at about 30 PeV and improve by 2 orders of magnitude over IceCube.  The radio array will build on the concept of RNO-G that serves as the R&D scale array (~10\% level) of the radio component. The design of this radio array was the result of a multi-year effort by the community, in the latest phase as an integral part of a planning effort of the IceCube-Gen2 collaboration includes the respective radio community.  



% \begin{figure}[tb]
% \begin{center}
% \includegraphics[width=1.0\textwidth]{SnowmassBook_IF/Instrumentation/IF10/figures/surface_geometry_tdr.pdf}
% \end{center}
% \caption{Top view of the envisioned IceCube-Gen2 Neutrino Observatory facility at the South Pole station, Antarctica. From left to right: The radio array consisting of 525 stations (shallow and hybrid).  IceCube-Gen2 strings in the optical high-energy array. 120 new strings (shown as orange points) are spaced 240 m apart and instrumented with 80 newly developed optical modules each, over a vertical length of 1.25 km. The total instrumented volume in this design is 7.9 times larger than the current IceCube detector array (blue points). On the far right, the layout for the seven IceCube Upgrade strings relative to existing IceCube strings is shown.}
% \label{fig:topview}
% \end{figure}



% The technological advancements in the optical array design:
% \begin{itemize}
%     \item Optical sensors: Contain 16 or 18 PMTs (directional 4 $\pi$ sensitivity, 3 x larger sensitivity of IceCube sensor)
%     \item New PMT of 4 inch size with short stem in development by two manufacturers
%     \item Optimized trigger and data acquisition scheme to allow factor 10 reduction in bandwidth, factor of 3 reduction in cables. 
%     \item integrated radio+scintillator air shower array on the footprint of the 5 km$^2$ optical array. 
%     \item more efficient drill and energy saving technology, including solar power. 
% \end{itemize}

% The technological advancements in the radio array design:

% \begin{itemize}
%     \item A hybrid radio array design building on developments of ARA, ARIANNA and RNO-G.  
%     \item New drill technology for fast drilling of holes for antennas down to 150\,m depth. 
%     \item possible use of autonomous power and wireless communication as tested in RNO-G.
% \end{itemize} 

% The integrated IceCube-Gen2 design is driven by the design requirement of sensitivity to a cosmic neutrino flux over a range from $10^3$ to $10^{10}$ GeV.  

% The following R&D opportunities have been identified for IceCube-Gen2:
% \begin{itemize}
%     \item Design of a new ASIC for the PMT signal readout (~100Msps, 12 bit, 2 channels). Given the large channel count of about 170,000 PMT channels, a significant cost and power saving could be realized. 
%     \item Design of an integrated readout chip could result in cost and power savings for radio DAQ systems.  
%  %   \item R\&D for further optimization of power and communications infrastructure. 
% \end{itemize}





%\paragraph{point to some examples with references}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%  If you would like to use BibTEX for the bibliography, please feel free to do so.  It is not required.

%  To use BibTeX,

%    1.  uncomment the following two lines,
%    2.  comment out everything below from  \begin{thebibliography}{99}   to \end{thebibliography).
%    3.  create the file  myreferences.bib in this directory, and process this file in the usual way

%\bibliographystyle{JHEP}
%\bibliography{Instrumentation/IF02/myreferences} 

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%










\section{Facilities}
\subsection{Calibration and test beam facilities}
Progress in particle physics depends on a multitude of unique facilities and capabilities that enable the advancement of detector technologies. Among these are test beams and irradiation facilities, which allow users to test the performance and lifetime of their detectors under realistic conditions. Test beam facilities are particularly important for collider and neutrino detector applications, while irradiation facilities are crucial for collider as well as some space-based astro particle detectors. It is important that the energy, intensity, particle composition and time structure of the beams are adequate for the detector needs for the next generation. In the area of irradiation facilities overlapping needs between detector and accelerator instrumentation as well as targetry development can be addressed.

\subsection{Low noise and environmentally stable facilities}
The particle physics community relies on a variety of specialized environmental conditions for operation of the most sensitive instrumentation. These include  low vibration/geologically quite environments, low electromagnetic interference environments, low radioactive background environments, and cryogenic environments to suppress thermal noise. Environmentally stable facilities, i.e. low vibration and/or low electromagnetic interference, tend to be very specialized for specific equipment (e.g. isolating a laser system or NMR) or to suppress specific frequency bands (seismic or electromagnetic) making it difficult to define the requirements for a general purpose user facility. In addition,these facilities are generally within the reach of individual research groups to establish locally as needed.

\subsection{Cryogenic Test Facilities}
Cryogenic test facilities are critical infrastructure for physics experiments in a variety of fields. Some notable examples include studying noble liquid properties for particle detection, low-temperature device development, and research in quantum information. The required technical knowledge and infrastructure capacity, including the cost of setting up and operating the test facilities, can place them out of reach of many individual group research groups. As such, these research areas would greatly benefit from centralized user facilities. Cryogenic test facilities can require significant investments in infrastructure and ongoing operations costs, and warrant consideration of the development of national user facilities. 

Several international institutions have established LAr test stands typically for specific purposes or experiments with limited measurement capabilities and access to the community. Some relatively large-sized facilities (more than 100 liters of LAr) include the ICARUS $\sim 50$ liter LArTPC at CERN~\cite{I9-Arneodo} with $\sim250$ liter LAr capacity, which is mainly used for ICARUS and DUNE detector electronics readout studies; the ArgonCube detector at University of Bern with $\sim1100$ liter LAr capacity, which is dedicated for pixel readout in LAr and DUNE’s modular detector study; and the Integrated Cryostat and Electronics Built for Experimental Research Goals (ICEBERG) at Fermilab with $\sim3000$ liter LAr capability, which is dedicated to DUNE cold electronics studies. As can be seen, these facilities are typically tied to the specific tasks that are not easily accessible as a user facility with the general purpose of R\&D, such as testing new devices and detector designs, studying noble liquid property, calibrating detector signal response, or studying light detector performance, etc. The necessary initial components for a community LAr test facility include a large cryostat with sufficient volume and drift distance, adequate cryogenic infrastructure for condensing and gas circulation, a purification system to remove impurities with high electron attachment, a purity monitoring system with gas analyzers, basic high voltage system and readout electronics for TPC measurements, a photon detection system to study scintillation light, and the accompanying DAQ system.

The operation of sensors and systems at ultra-low temperature is a major growth field, but one which necessarily has a high barrier for entry due to the relatively high cost of equipment, not just for the cooling platform itself but also associated measurement equipment and electronics and a knowledge gap in the operation and engineering of devices and systems at cryogenic temperatures. In addition, the typical fabrication, measurement and analysis cycle associated with the development of cryogenic devices will often mean that test stands can be idle for considerable periods of time, making the economics of every PI or research group having dedicated research facilities economically unattractive.
The establishment of a centralized facility would democratize the process of device development by allowing users access to test stands and measurement equipment for a variety of different tests, including but not limited to thermal, RF and low frequency tests. This is particularly valuable at the pre-proposal and proof-of-concept stages to validate new ideas before committing to full proposals or the expense of purchasing dedicated test equipment. In addition, such a facility would serve as a repository of knowledge of low temperature materials and other specialized information and offer a medium to connect researchers with specialized cryogenic engineering resources. Finally, such a facility is a vital tool for training a future workforce by providing hands-on experience in the operation of cryogenic systems and measurement equipment, typically outside the ability of a University level teaching laboratory to provide.
Such a facility would necessarily consist of more than a single refrigerator test stand, since this is something that a well-equipped PI laboratory would be able to provide. Instead, it is envisaged that the proposed User Facility would provide a suite of test stands available for different experiment types, including a number of test stands providing environments for the testing of specialized devices such underground and low-background environments, test stands with optical access, and stands incorporating magnetic fields.


\section{Synergies}
\subsection{Collaborative research models}
The U.S. HEP model for these has been to base facilities and core capabilities at national labs as user facilities funded by KA-25. Alternative approaches might be considered based on models such as the the CERN RD research programs or the NNSA NA-20 research consortia. The CERN RD programs provide an organizational framework within which collaborative research is conducted, but provide no direct funding support. However, engagement in these RD programs often provides a strong argument for grant funding to support participation. In contract, the NA-20 research consortia are multi-year multi-institutional research proposals with funding provided to the university groups and an expectation of support from national laboratories already funded by the office. In both cases, the intent is to build 5+ year programs of research to address larger programmatic ambitions than individual institutions could tackle.The HEP investment in LAPPDs was to a large extent such a program.

\subsection{Multidisciplinary research}
The topic of multidisciplinary R\&D was explored in the MultiHEP 2020 workshop, held virtually on Nov. 9-12, 2020. This consisted of a series of invited presentations and panel discussions to collect experience on successes, challenges, and lessons about multi-disciplinary collaborations to further High Energy Physics R&D.  The focus is on HEP developments that make use of expertise from outside HEP through collaborative efforts.  R\&D disciplines explored included chemistry, materials science, nuclear science, micro and nano fabrication. Examples included small efforts at universities, projects at labs, work with industry through SBIR and otherwise, long-term multi-institute development such as LAPPD, and agency experience. The workshop panel discussions identified relevant points in the categories working with other fields, working with industry, and multidisciplinary personnel and funding.

\paragraph{Working with other fields}
Development of new instrumentation is often only possible through expertise and capabilities from outside HEP. Examples at the workshop were LAPPD, barium tagging for 0$\nu\beta\beta$ decay, use of carbon nanotubes for photon detection, etc. The following observations were collected:
\begin{itemize}
    \item Informal discussions are required to establish work scope for reasons summarized as ``because you don't know what you don't know''.
    \item Some interest in the HEP goals is more important than expert standing in another field. 
    \item 
    Research philosophy is different in other fields. in HEP negative results are a success (most HEP results are negative!) Other fields have narrowly defined goals and positive results are the measure of success.
    \item Publication approach is different in other fields. No preprints: scoops common so results remain secret till published. Publications are geared to the next funding proposal. Author lists are small. It's a good idea to have agreements formalizing collaboration, funding, author lists etc. after initial informal discussions.  
\end{itemize}

\paragraph{Working with industry}
There were numerous reports about successful SBIR efforts. The SBIR program offers a good path to fund multidisciplinary development by partnering with an appropriate firm. True partnerships between HEP scientists and firms are essential for success. An issue with SBIR is that many technologies critical for HEP do not have a lucrative commercialization path, but SBIR requires commercialization as the end product of Phase 2. Even when commercialization is in principle possible, there is a large gap between phase 2 and volume production for profit. It is difficult for small companies to bridge that gap. 

Connecting with the right company is a challenge. Networking efforts can help. NP holds an annual exchange meeting for this purpose. Some national labs have industry days, but not regularly or at the same level. BNL has a discovery park incubator. 

For multidisciplinary work there may be co-founding opportunities. Each office has to allocate and spend the required SBIR levels and this leads to roundoff errors becasue each office has to spend down an exact amount. This would allows NP to co-fund something with HEP, for example.  

\paragraph{Multidiscpiplinary personnel and funding}
\begin{itemize}
    \item Few institutes train people in multiple disciplines at once. It is therefore hard to recruit people to carry out multidisciplinary work.
    \item The other side of the coin is that a student or postdoc developing in two disciplines at once may have a hard time finding the next job, because they will not be competitive in either one of these disciplines with peers who devoted themselves fully to it. They need to find a job where both disciplines are required. 
    \item Funding agency offices tend to not like paying for personnel normally under other offices, which makes it hard to find multidisciplinary work with a single grant. Recent QIS and Micrelectronics FOAs have aimed at multidisciplinary work. Microelectronics has been more successful because (unusually) multiple offices co-funded the same FOA, while this was not the case for QIS, where each office had separate FOAs. More funding like Microelectronics is needed if fostering multidisciplinary work is desired.    
\end{itemize}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%  If you would like to use BibTEX for the bibliography, please feel free to do so.  It is not required.

%  To use BibTeX,

%    1.  uncomment the following two lines,
%    2.  comment out everything below from  \begin{thebibliography}{99}   to \end{thebibliography).
%    3.  create the file  myreferences.bib in this directory, and process this file in the usual way

\bibliographystyle{JHEP}
\bibliography{Instrumentation/InstrumentationReferences} 

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


%\begin{thebibliography}{99}

%\input Instrumentation/bibliography.tex

%\end{thebibliography}

==> Instrumentation/bibliography.tex <==

\bibitem{I4-Scoresby}
J. Scoresby, ``Journals'', 1820.

\bibitem{I-Beale}
A. Beale, ``Surgical Writings'', 1839.



==> tcilcomm.tex <==
% Macros used for TCI styles released with Scientific Word 1.1.
%Copyright (C) 1992-93 TCI Software Research, Inc.
\typeout{TCILCOMM Macros for TCI styles <08 Apr 93>.}
%
% Revisions:
% 08 Apr 93 - GP change line length to under 80 characters
% 30 Mar 92 - AO added \setmoremathsizes and hooks to, e.g. \@xpt,
%             for support of bold Greek
%
%%ltg added this to try to get 12pt to come through
%\DeclareOption{12pt}{\renewcommand\@ptsize{2}}
%%end ltg

\def\@ptoptions{%
 \let\@elt\relax\@for\@tempa:=\@optionlist\do{%
  \expandafter\let\expandafter\@tempb\csname ds@\@tempa\endcsname
  \expandafter\let\expandafter\@tempc\csname ds@11pt\endcsname
  \ifx\@tempb\@tempc\else
   \expandafter\let\expandafter\@tempc\csname ds@12pt\endcsname
   \ifx\@tempb\@tempc\else\let\@tempb\relax\fi
   \fi
  \@tempb
  }%
 }%
%
% read in style file, but only process the pt size options
%
\def\@ptoptinput#1{%
 \let\@save@optionlist\@optionlist
 \let\@save@options\@options
 \let\@options\@ptoptions
 %
 \input #1
 %
 \let\@optionlist\@save@optionlist
 \let\@options\@save@options
 }%
%
% the <21 Feb 92> version of letter.sty requires:
\ifx\undefined\reset@font
 \def\reset@font{}%
 \fi
%
% Change LaTeX
%
% Add command to append tokens
\newtoks\@temptokenb
\long\def\appdef#1#2{%
 \ifx#1\undefined\let#1\@empty\fi
 \@temptokena\expandafter{#1}\@temptokenb{#2}%
 \edef#1{\the\@temptokena\the\@temptokenb}%
 }%
\long\def\prepdef#1#2{%
 \ifx#1\undefined\let#1\@empty\fi
 \@temptokena\expandafter{#1}\@temptokenb{#2}%
 \edef#1{\the\@temptokenb\the\@temptokena}%
 }%
% Discard contents of \box\@cclv at beginning of document
\appdef\document{{\output{\setbox\z@\box\@cclv}\endgraf\null\eject}}%
% Fix mark register expansion
\def\leftmark{\expandafter\@leftmark\botmark{}{}{}\@nil}%
\def\rightmark{\expandafter\@rightmark\firstmark{}{}{}\@nil}%
\def\@leftmark#1#2#3\@nil{#1}%
\def\@rightmark#1#2#3\@nil{#2}%
%
%\show\raggedright
\newskip\raggedglue
\raggedglue\z@ plus20\p@ minus\z@
\def\raggedright{%
 \let\\=\@centercr\@rightskip\raggedglue\rightskip
 \@rightskip\leftskip\z@\parindent\z@
 }%
%
\def\@centercr{%
 \ifhmode\unskip\else\@badcrerr\fi\@@par
 \@ifstar{\penalty\@M\@xcentercr}{\@xcentercr}%
 }%
%
\def\traceoutput{\tracingoutput2\showboxbreadth\maxdimen
 \showboxdepth\maxdimen}%
%
\newcount\@hour\newcount\@minute\chardef\@x10\chardef\@xv60
\def\@time{%
  \@minute\time\@hour\@minute\divide\@hour\@xv
  \ifnum\@hour<\@x 0\fi\the\@hour:%
  \multiply\@hour\@xv\advance\@minute-\@hour
  \ifnum\@minute<\@x 0\fi\the\@minute
  }%
%
% change \@array to allow \par to mean something within its scope
%
\def\@array [#1]#2{%
 \setbox\@arstrutbox\hbox{\vrule height\arraystretch\ht
  \strutbox depth\arraystretch\dp\strutbox width\z@}%
 \@mkpream{#2}%
 \edef\@preamble{\halign\noexpand\@halignto\bgroup\tabskip
  \z@\@arstrut\@preamble\tabskip\z@\cr}%
 \let\@startpbox\@@startpbox\let\@endpbox\@@endpbox
 \if#1t\vtop\else\if#1b\vbox\else\vcenter\fi\fi
 \bgroup
  %\let\par\relax
  \let\@sharp##
  \let\protect\relax
  \lineskip\z@\baselineskip\z@
  \@preamble
 }%
%
% Expands to hex digit corresponding to the value of the argument
%
\def\hexnumber@#1{\ifnum#1<10 \number#1\else
 \ifnum#1=10 A\else\ifnum#1=11 B\else\ifnum#1=12 C\else
 \ifnum#1=13 D\else\ifnum#1=14 E\else\ifnum#1=15 F\fi\fi\fi\fi\fi\fi\fi}%
%
% define command to set more math sizes.
% Styles like Greekbf will hook in here.
%
\def\setmoremathsizes#1#2#3{}%
%
% define size switch addenda
%  Note: these choices agree with those in lfonts.tex, even if incorrect.
%
\prepdef\@vpt{\setmoremathsizes{fiv}{fiv}{fiv}}%
\prepdef\@vipt{\setmoremathsizes{six}{six}{six}}%
\prepdef\@viipt{\setmoremathsizes{sev}{fiv}{fiv}}%
\prepdef\@viiipt{\setmoremathsizes{egt}{six}{fiv}}%
\prepdef\@ixpt{\setmoremathsizes{nin}{six}{fiv}}%
\prepdef\@xpt{\setmoremathsizes{ten}{sev}{fiv}}%
\prepdef\@xipt{\setmoremathsizes{elv}{egt}{six}}%
\prepdef\@xiipt{\setmoremathsizes{twl}{egt}{six}}%
\prepdef\@xivpt{\setmoremathsizes{frtn}{ten}{sev}}%
\prepdef\@xviipt{\setmoremathsizes{svtn}{twl}{ten}}%
\prepdef\@xxpt{\setmoremathsizes{twty}{frtn}{twl}}%
\prepdef\@xxvpt{\setmoremathsizes{twty}{twty}{svtn}}%
%
% The \newfield command defines (like \newenvironment) a user syntax:
%
%   \newfield{foo}
%
% lets you write
%
%   \begin{foo}...\end{foo}
%
% but differs from \newenvironment in that TeX parses the entire content
% of the field and stores it in a macro \the@foo, and then executes \@do@foo.
%
% This means that the content of the field is actually more like an argument
% than the content of an environment. So \verb will not necessarily work
% within a field, and neither will \index. Caveat emptor.
%
% The default procedure for a field is to process its argument within a
% group.  If you want a field to simply store its data away, define its
% procedure to be synonymous with \@empty, as illustrated below.
%
\long\def\@readenvir#1#2\end{%
 \appdef\envirsofar{#2}%
 \@ifnextchar\bgroup{\@checkenvir{#1}}{\@envirenderr}%
 }%
%
\def\@envirenderr{%
 \@latexerr{\string\end\space not followed by environment name}\@eha
 }%
%
\def\@checkenvir#1#2{%
 \def\@tempa{#1}\def\@tempb{#2}%
 \ifx\@tempa\@tempb
  \ifx\envirsofar\@blankspace\let\envirsofar\@empty\fi
  \expandafter\let\csname the@#1\endcsname\envirsofar
  \def\@tempa{\csname @do@#1\endcsname}%
  \else
  \appdef\envirsofar{\end{#2}}%
  \def\@tempa{\@readenvir{#1}}%
  \fi
 \@tempa
 }%
%
\def\newfield#1#2{%
 \expandafter\@ifdefinable\csname#1\endcsname{%
  \expandafter\def\csname#1\endcsname{%
   \endgroup\let\envirsofar\@empty\@readenvir{#1}%
   }%
  \expandafter\let\csname the@#1\endcsname\@empty
  \expandafter\ifx\csname @do@#1\endcsname\relax
   \expandafter\def\csname @do@#1\endcsname{{\csname the@#1\endcsname}}%
   \fi
  }%
 }%
%
\def\@blankspace{ }% SciWord's nil field
%
\def\letparBL{\def\par{\\}}%
\def\letparSP{\def\par{\ }}%
\def\letparQD{\def\par{\quad}}%
\def\letparSL{\def\par{\hbox to1em{\hfil/\hfil}}}%
%
% When \par is processed in the page head, gobble up the rest of the
% argument.
\def\@gobblepar#1\@empty{}%
%
% Physical page size after trim
\newdimen\trimwidth
\newdimen\trimheight
\newdimen\botmargin
\newdimen\marginpartotal
%
\def\adjustpagemargin{% adjust \oddsidemargin by \marginpartotal
 \marginpartotal\marginparwidth\advance\marginpartotal\marginparsep
 \advance\oddsidemargin\marginpartotal
 }%
%
\def\settextheight{% calculate textheight constrained by:
 \textheight\trimheight
 \advance\textheight-\topmargin
 \advance\textheight-\headheight
 \advance\textheight-\headsep
 \advance\textheight-\footskip
 \advance\textheight-\botmargin
 }%
%
\def\vcenterpagemargin{% calculate \topmargin constrained by:
 \topmargin\trimheight
 \advance\topmargin-\textheight
 \advance\topmargin-\headheight
 \advance\topmargin-\headsep
 \advance\topmargin-\footskip
 \divide\topmargin\tw@\botmargin\topmargin
 }%
%
\def\centerpagemargin{% calculate \oddsidemargin constrained by:
 \oddsidemargin\trimwidth
 \advance\oddsidemargin-\textwidth
 \advance\oddsidemargin-\marginparwidth
 \advance\oddsidemargin-\marginparsep
 \divide\oddsidemargin\tw@
 \evensidemargin\oddsidemargin
 \adjustpagemargin
 }%
%
\def\leftpagemargin{% calculate \oddsidemargin constrained by:
 \oddsidemargin\trimwidth
 \advance\oddsidemargin-\textwidth
 \advance\oddsidemargin-\marginparwidth
 \advance\oddsidemargin-\marginparsep
 \advance\oddsidemargin-\evensidemargin
 \adjustpagemargin
 }%

